Extending Multi-Sense Word Embedding to Phrases and Sentences for Unsupervised Semantic Applications

Most unsupervised NLP models represent each word with a single point or single region in semantic space, while the existing multi-sense word embeddings cannot represent longer word sequences like phrases or sentences. We propose a novel embedding method for a text sequence (a phrase or a sentence) where each sequence is represented by a distinct set of multi-mode codebook embeddings to capture different semantic facets of its meaning. The codebook embeddings can be viewed as the cluster centers which summarize the distribution of possibly co-occurring words in a pre-trained word embedding space. We introduce an end-to-end trainable neural model that directly predicts the set of cluster centers from the input text sequence during test time. Our experiments show that the per-sentence codebook embeddings significantly improve the performances in unsupervised sentence similarity and extractive summarization benchmarks. In phrase similarity experiments, we discover that the multi-facet embeddings provide an interpretable semantic representation but do not outperform the single-facet baseline.

==> AAAI 2021 NSD/BERT_large.tex <==
\begin{table}[t!]
\centering
\scalebox{0.9}{
\begin{tabular}{|c|c|c|c|}
\hline
Method & Hidden size & \#Parameters & Testing Time \\ \hline
K=1 & 300 & 6.7M & 9 ms \\
K=10 & 300 & 13.7M & 18 ms \\
BERT Base & 768 & 86.0M & 18 ms \\
BERT Large & 1024 & 303.9M & 65 ms \\ \hline
\end{tabular}
}
\centering
\caption{Comparison of model sizes. The number of parameters does not include the word embedding layer. We show the test time required for a batch with 50 sentences using one 1080Ti GPU.}
\label{tb:model_size}
\end{table}

\begin{table*}[t!]
\centering
\begin{minipage}{.5\linewidth}
\centering
\scalebox{0.9}{
\begin{tabular}{|cc|cc|cc|}
\hline
\multicolumn{2}{|c|}{Method} & \multicolumn{2}{|c|}{Dev} & \multicolumn{2}{|c|}{Test} \\ \hline
\multicolumn{1}{|c|}{Model} & Score & All & Low & All & Low   \\ \hline
%BERT Base & \multicolumn{1}{|c|}{Avg} &62.3 & 42.1 & 51.2 & 39.1 \\ \hline
%BERT Large & \multicolumn{1}{|c|}{Avg} & 68.4 & 52.6 & 59.5 & 49.4 \\ \hline
BERT Base & \multicolumn{1}{|c|}{Prob\_avg} &72.1 & 57.0 & 57.8 & 55.1 \\ 
BERT Large & \multicolumn{1}{|c|}{Prob\_avg} & 74.3 & 61.0 & 65.0 & \textbf{60.0} \\ \hline
\multirow{2}{*}{Our a (GloVe) K10} & \multicolumn{1}{|c|}{Prob\_avg} & 72.0 & 60.5 & 61.4 & 59.3 \\ 
& \multicolumn{1}{|c|}{Prob\_WMD} & \textbf{76.2} & \textbf{62.6} & \textbf{66.1} & 58.1 \\ \hline
\end{tabular}
}
\caption{Compare BERT Large with Ours in Table~\reftbsts%~\ref{tb:STS}
.}
\label{tb:STS_bert}
\end{minipage}%
\quad 
\begin{minipage}{.48\linewidth}
\centering
\scalebox{1}{
\begin{tabular}{|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{Method} & R-1 & R-2 & Len \\ \hline
\multirow{2}{*}{BERT Base} & W Emb & 31.2 & 11.2 & 44.9 \\ 
 & Sent Emb  & 32.3  & 10.6 & 91.2 \\ \hline 
\multirow{2}{*}{BERT Large} & W Emb & 31.1 &	11.0 & 46.8 \\ 
 & Sent Emb  & 32.7 & 10.9 & 86.5 \\ \hline
Our c (K=100) & Bases & \textbf{35.0} & \textbf{12.8} & 92.9 \\ \hline

\end{tabular}
}
\caption{Compare BERT Large with Ours in Table~\reftbsum .}
\label{tb:sum_bert}
\end{minipage}
\end{table*}

\begin{table*}[t!]
\scalebox{0.8}{
\begin{tabular}{|cc|cc|c|c|c|c|c|c|c|}
\hline
& & \multicolumn{7}{|c|}{Lowercased} & \multicolumn{2}{|c|}{Uppercased} \\ \cline{3-11}
\multicolumn{2}{|c|}{Method} & \multicolumn{2}{c|}{SemEval} & Turney (5) & Turney (10) & BiRD & WikiSRS-Sim & WikiSRS-Rel & WikiSRS-Sim & WikiSRS-Rel  \\ \hline %\cline{1-2}
\multicolumn{1}{|c|}{Model} & Score & AUC & F1 & Acc & Acc & Pearson & \multicolumn{4}{|c|}{Spearman}  \\ \hline
BERT Base & \multicolumn{1}{|c|}{Avg} & 66.5 & 67.1 & 43.4 & 24.3 & 44.4 & 43.3 & 40.7 & 40.3 &	37.8  \\ 
BERT Large & \multicolumn{1}{|c|}{Avg} & 72.4 & 66.7 & \textbf{51.3} & 32.1 & 47.5 & 49.6 & 48.1 & 28.6 & 34.0  \\ 
Ours (K=1) & \multicolumn{1}{|c|}{Emb} & \textbf{87.8} & \textbf{78.6} & 50.3 & \textbf{32.5} & \textbf{60.6} & \textbf{67.1} & \textbf{65.8} & \textbf{69.4} &	\textbf{69.4} \\ \hline
\end{tabular}
}
\centering
\caption{Compare BERT Large with Ours in Table~\reftbphrase%~\ref{tb:phrase_sim}
. }
\label{tb:phrase_sim_bert}
%$\dagger$The results are taken from~\citet{WikiSRS}.   }
\end{table*}


\begin{table}[t!]
\centering
\scalebox{1}{
\begin{tabular}{|c|cc|cc|}
\hline
\multirow{2}{*}{Method} & \multicolumn{2}{|c|}{Dev} & \multicolumn{2}{|c|}{Test}  \\ \cline{2-5}
& AUC & Acc  & AUC & Acc \\ \hline
BERT Base (Avg) & 25.6 & 50 & 25.6 & 50 \\ 
BERT Large (Avg) & 20.2 & 50  & 20.1  & 50 \\ 
Ours (K=1) & \textbf{29.3} & \textbf{82.7} & \textbf{29.6}  & \textbf{81.0} \\ \hline
\end{tabular}
}
\centering
\caption{Compare BERT Large with Ours in Table~\ref{tb:phrase_hyper}.}
\label{tb:phrase_hyper_bert}

\end{table}





==> AAAI 2021 NSD/color_map.tex <==
\definecolor{c00}{rgb}{1 0.00 0.00}
\definecolor{c01}{rgb}{1 0.01 0.01}
\definecolor{c02}{rgb}{1 0.02 0.02}
\definecolor{c03}{rgb}{1 0.03 0.03}
\definecolor{c04}{rgb}{1 0.04 0.04}
\definecolor{c05}{rgb}{1 0.05 0.05}
\definecolor{c06}{rgb}{1 0.06 0.06}
\definecolor{c07}{rgb}{1 0.07 0.07}
\definecolor{c08}{rgb}{1 0.08 0.08}
\definecolor{c09}{rgb}{1 0.09 0.09}
\definecolor{c10}{rgb}{1 0.10 0.10}
\definecolor{c11}{rgb}{1 0.11 0.11}
\definecolor{c12}{rgb}{1 0.12 0.12}
\definecolor{c13}{rgb}{1 0.13 0.13}
\definecolor{c14}{rgb}{1 0.14 0.14}
\definecolor{c15}{rgb}{1 0.15 0.15}
\definecolor{c16}{rgb}{1 0.16 0.16}
\definecolor{c17}{rgb}{1 0.17 0.17}
\definecolor{c18}{rgb}{1 0.18 0.18}
\definecolor{c19}{rgb}{1 0.19 0.19}
\definecolor{c20}{rgb}{1 0.20 0.20}
\definecolor{c21}{rgb}{1 0.21 0.21}
\definecolor{c22}{rgb}{1 0.22 0.22}
\definecolor{c23}{rgb}{1 0.23 0.23}
\definecolor{c24}{rgb}{1 0.24 0.24}
\definecolor{c25}{rgb}{1 0.25 0.25}
\definecolor{c26}{rgb}{1 0.26 0.26}
\definecolor{c27}{rgb}{1 0.27 0.27}
\definecolor{c28}{rgb}{1 0.28 0.28}
\definecolor{c29}{rgb}{1 0.29 0.29}
\definecolor{c30}{rgb}{1 0.30 0.30}
\definecolor{c31}{rgb}{1 0.31 0.31}
\definecolor{c32}{rgb}{1 0.32 0.32}
\definecolor{c33}{rgb}{1 0.33 0.33}
\definecolor{c34}{rgb}{1 0.34 0.34}
\definecolor{c35}{rgb}{1 0.35 0.35}
\definecolor{c36}{rgb}{1 0.36 0.36}
\definecolor{c37}{rgb}{1 0.37 0.37}
\definecolor{c38}{rgb}{1 0.38 0.38}
\definecolor{c39}{rgb}{1 0.39 0.39}
\definecolor{c40}{rgb}{1 0.40 0.40}
\definecolor{c41}{rgb}{1 0.41 0.41}
\definecolor{c42}{rgb}{1 0.42 0.42}
\definecolor{c43}{rgb}{1 0.43 0.43}
\definecolor{c44}{rgb}{1 0.44 0.44}
\definecolor{c45}{rgb}{1 0.45 0.45}
\definecolor{c46}{rgb}{1 0.46 0.46}
\definecolor{c47}{rgb}{1 0.47 0.47}
\definecolor{c48}{rgb}{1 0.48 0.48}
\definecolor{c49}{rgb}{1 0.49 0.49}
\definecolor{c50}{rgb}{1 0.50 0.50}
\definecolor{c51}{rgb}{1 0.51 0.51}
\definecolor{c52}{rgb}{1 0.52 0.52}
\definecolor{c53}{rgb}{1 0.53 0.53}
\definecolor{c54}{rgb}{1 0.54 0.54}
\definecolor{c55}{rgb}{1 0.55 0.55}
\definecolor{c56}{rgb}{1 0.56 0.56}
\definecolor{c57}{rgb}{1 0.57 0.57}
\definecolor{c58}{rgb}{1 0.58 0.58}
\definecolor{c59}{rgb}{1 0.59 0.59}
\definecolor{c60}{rgb}{1 0.60 0.60}
\definecolor{c61}{rgb}{1 0.61 0.61}
\definecolor{c62}{rgb}{1 0.62 0.62}
\definecolor{c63}{rgb}{1 0.63 0.63}
\definecolor{c64}{rgb}{1 0.64 0.64}
\definecolor{c65}{rgb}{1 0.65 0.65}
\definecolor{c66}{rgb}{1 0.66 0.66}
\definecolor{c67}{rgb}{1 0.67 0.67}
\definecolor{c68}{rgb}{1 0.68 0.68}
\definecolor{c69}{rgb}{1 0.69 0.69}
\definecolor{c70}{rgb}{1 0.70 0.70}
\definecolor{c71}{rgb}{1 0.71 0.71}
\definecolor{c72}{rgb}{1 0.72 0.72}
\definecolor{c73}{rgb}{1 0.73 0.73}
\definecolor{c74}{rgb}{1 0.74 0.74}
\definecolor{c75}{rgb}{1 0.75 0.75}
\definecolor{c76}{rgb}{1 0.76 0.76}
\definecolor{c77}{rgb}{1 0.77 0.77}
\definecolor{c78}{rgb}{1 0.78 0.78}
\definecolor{c79}{rgb}{1 0.79 0.79}
\definecolor{c80}{rgb}{1 0.80 0.80}
\definecolor{c81}{rgb}{1 0.81 0.81}
\definecolor{c82}{rgb}{1 0.82 0.82}
\definecolor{c83}{rgb}{1 0.83 0.83}
\definecolor{c84}{rgb}{1 0.84 0.84}
\definecolor{c85}{rgb}{1 0.85 0.85}
\definecolor{c86}{rgb}{1 0.86 0.86}
\definecolor{c87}{rgb}{1 0.87 0.87}
\definecolor{c88}{rgb}{1 0.88 0.88}
\definecolor{c89}{rgb}{1 0.89 0.89}
\definecolor{c90}{rgb}{1 0.90 0.90}
\definecolor{c91}{rgb}{1 0.91 0.91}
\definecolor{c92}{rgb}{1 0.92 0.92}
\definecolor{c93}{rgb}{1 0.93 0.93}
\definecolor{c94}{rgb}{1 0.94 0.94}
\definecolor{c95}{rgb}{1 0.95 0.95}
\definecolor{c96}{rgb}{1 0.96 0.96}
\definecolor{c97}{rgb}{1 0.97 0.97}
\definecolor{c98}{rgb}{1 0.98 0.98}
\definecolor{c99}{rgb}{1 0.99 0.99}
\definecolor{c100}{rgb}{1 1.00 1.00}

==> AAAI 2021 NSD/conclusion.tex <==
In this work, we propose a framework for learning the co-occurring distribution of the words surrounding a sentence or a phrase.
%overcome the computational and sampling efficiency challenges of learning the multi-facet representation for phrases or sentences. 
Even though there are usually only a few words that co-occur with each sentence, we demonstrate that the proposed models can learn to predict interpretable cluster centers conditioned on an (unseen) sentence.

In the sentence similarity tasks, the results indicate that the similarity between two sets of multi-facet embeddings well correlates with human judgments, and we can use the multi-facet embeddings to estimate the word importance and improve various widely-used similarity measurements in a pre-trained word embedding space such as GloVe. In a single-document extractive summarization task, we demonstrate multi-facet embeddings significantly outperform classic unsupervised sentence embedding or individual word embeddings. 
%when the first few sentences are not assumed to be a good summary. 
Finally, the results of phrase similarity tasks suggest that a single embedding might be sufficient to represent the co-occurring word distribution of a phrase.

%especially when the pair of sentences are significantly different from each other.
%low 
%and the representation outperforms widely-used baselines such as BERT, skip-thoughts and various approaches based on GloVe in several unsupervised benchmarks. 
%The experimental results also suggest that multi-facet embeddings perform the best when the input sequence (e.g., a sentence) involves many aspects, while multi-facet and single-facet embeddings perform similarly good when the input sequence (e.g., a phrase) usually involves only one aspect. 

%We use a neural encoder to model the compositional meaning of the target sequence and use a neural decoder to predict a set of codebook embeddings as the representation of the sentences or phrases. During training, we use a non-negative sparse coefficient matrix to dynamically match the predicted codebook embeddings to a set of observed co-occurring words and allow the neural decoder to predict the clustering centers with an arbitrary permutation. 



%In the future, we would like to train a single model which could generate multi-facet embeddings for both phrases and sentences, and evaluate the method as a pre-trained embedding approach for supervised or semi-supervised settings. Furthermore, we plan to apply this method to other unsupervised learning tasks that heavily rely on co-occurrence statistics such as graph embedding or recommendation.
%since this approach is totally unsupervised, 

%apply this model to several  applications. 

%coding loss to  match
%allow the neural network to predict 

%The predict codebook vectors are matched with co-occuring

%we focus on evaluating the performance of the models in unsupervised applications 
%Pretrained embedding



%For each of the applications, we are aware of some other unsupervised approaches (such as FCT for phrase similarity, DIVE for hypernym detection, TextRank for summarization). We will compare our methods with them after controlling the training corpus and pre-processing step.

%In future work, we should list some other unsupervised baseline (specifically for certain applications) we want to compare with more fairly. Such as FCT, TextRank, skip-thoughts? BERT?

%Know what property in the distributional semantic space we should have in order to make the model fit well

%, skip-thoughts for sentence similarity

==> AAAI 2021 NSD/exp_details.tex <==


%Training deep neural network on a large raw corpus takes time. Due to our resources constraint, we allow our model to use only one modern GPU and being trained for one week. 
%, and we find that the model still underfits the training data after converge (i.e., the training loss and validation loss are similar).


\subsection{Training}
The training algorithm of non-negative sparse coding (NNSC) loss can be seen in Algorithm~\ref{algo:NNSC}. Given the computational resource constraints, we keep our model simple enough to have the  training loss nearly converged after 1 or 2 epoch(s). Since training takes a long time, we do not fine-tune the hyper-parameters in our models. We use a much smaller model than BERT but the architecture details in our transformer and most of its hyper-parameters are the same as those used in BERT. 

The sparsity penalty weights on coefficient matrix $\lambda$ in~\refeqer is set to be 0.4. The maximal sentence size is set to be 50, and we ignore the sentences longer than that. The maximal number of co-occurring words is set to be 30 (after removing the stop words), and we sub-sample the words if there are more words in the previous and next sentence. All words occurring less than 100 times in the training corpus are mapped to <unk>.

The number of dimensions in transformers is set to be 300. For sentence representation, dropout on attention is 0.1. Its number of transformer layers on the decoder side is 5 for $K = 10$, and the number of transformer layers on the decoder side is set to be 1 for $K = 1$ because we do not need to model the dependency of output codebook embeddings. For phrase representation, the number of transformer layers on the decoder side is 2, and the dropout on attention is 0.5. %The window size $d_t^1=d_t^2$ is set to be 5.  and 
%We will release the code to reveal more hyper-parameter setting details.

%We remove multi-head attention layer in decoder that uses contextualized word embedding from the encoder (i.e., the architecture of our decoder for phrase is the same as BERT transformer encoder). 

All the architecture and hyperparameters (except the number of codebook embeddings) in our models are determined by the validation loss of the self-supervised co-occurring word reconstruction task in \refeqobj. The number of codebook embeddings $K$ is chosen by the performance of training data in each task, but we observe that the performances are usually not sensitive to the numbers as long as $K$ is large enough as shown in our phrase experiments. Furthermore, we suspect that the slight performance drops of models with too large $K$ might just be caused by the fact that larger $K$ needs longer training time and 1 week of training is insufficient to make the model converge.
%We also suspect that training the model with larger K longer might eventually perform 

We use RegexpParser in NLTK~\citep{bird2009natural} to detect the phrase boundary. We use the grammar \textit{NP: {<JJ.*>*<VBG>*<NN.*>+}}. The sentence boundaries are detected using the rule-based pipeline in spaCy\footnote{\url{spacy.io/}} and POS tags are also detected using spaCy.

The lowercased list we use for removing stop words includes \textit{@-@, =, <eos>, <unk>, disambiguation, etc, etc., --, @card@, $\sim$, -, \_, @, \^, \&, *, <, >, (, ), \textbackslash, |, \{, \}, ], [, :, ;, ', ", /, ?, !, ,, ., 't, 'd, 'll, 's, 'm, 've, a, about, above, after, again, against, all, am, an, and, any, are, aren, as, at, be, because, been, before, being, below, between, both, but, by, can, cannot, could, couldn, did, didn, do, does, doesn, doing, don, down, during, each, few, for, from, further, had, hadn, has, hasn, have, haven, having, he, her, here, here, hers, herself, him, himself, his, how, how, i, if, in, into, is, isn, it, it, its, itself, let, me, more, most, mustn, my, myself, no, nor, not, of, off, on, once, only, or, other, ought, our, ours, ourselves, out, over, own, same, she, should, shouldn, so, some, such, than, that, the, their, theirs, them, themselves, then, there, these, they, this, those, through, to, too, under, until, up, very, was, wasn, we, were, weren, what, when, where, which, while, who, whom, why, with, won, would, wouldn, you, your, yours, yourself, yourselves}.


\begin{algorithm*}[!t]
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{Training corpus, sequence boundaries, and pre-trained word embedding.}
\Output{$F$}
Initialize $F$ \\
\ForEach{$I_t, \bm{W(N_t)}, \bm{W(N_{r_t})}$ \text{in training corpus}}{%
	Run forward pass on encoder and decoder to compute $\bm{F(I_t)}$ \\
	Compute $\bm{M^{O_t}} = \argmin_{\bm{M}} ||\bm{F(I_t)}\bm{M} - \bm{W(N_t)}||^2 + \lambda || \bm{M} ||_1 \forall k,j, \; 0 \leq \bm{M}_{k,j} \leq 1$,  \\
	Compute $\bm{M^{R_t}} = \argmin_{\bm{M}} ||\bm{F(I_t)}\bm{M} - \bm{W(N_{r_t})}||^2 + \lambda || \bm{M} ||_1 \forall k,j, \; 0 \leq \bm{M}_{k,j} \leq 1$, \\
	Run forward pass to compute $L_t$ in \refeqobj \\
	Treat $\bm{M^{O_t}}$ and $\bm{M^{R_t}}$ as constants, update $F$ by backpropagation
}
 \caption{Training using NNSC loss}
 \label{algo:NNSC}
\end{algorithm*}

\subsection{Testing}
The dataset sizes for sentence representation and phrase representation are summarized in Table~\ref{tb:dataset_size_sent} and Table~\ref{tb:dataset_size_phrase}, respectively. In our phrase experiments, we report the test sets of SemEval 2013 and Turney. For Turney dataset, we follow the evaluation setup of~\citet{fct, huang2017learning}, which ignores two unigram candidates being contained in the target phrase, because the original setup~\citep{turney2012} is too difficult for unsupervised methods to get a meaningful score (e.g., the accuracy of \textbf{GloVe Avg} is 0 in the original setting).
%have training and testing split and the performances in test sets are reported.

%We use the pre-trained model for BERT and ELMo. 
For skip-thoughts, the hidden embedding size is set to be 600. To make the comparison fair, we retrain the skip-thoughts in Wikipedia 2016 for 2 weeks.
%Due to the submission deadline, we only train skip-thoughts for 5 days.






==> AAAI 2021 NSD/experiments.tex <==

Quantitatively evaluating the quality of our predicted cluster centers is difficult because the existing label data and metrics are built for global clustering. The previous multi-sense word embedding studies often show that multiple embeddings could improve the single word embedding in the unsupervised word similarity task to demonstrate its effectiveness. Thus, our goal of experiments is to discover when and how the multi-facet embeddings can improve the similarity measurement in various unsupervised semantic tasks upon the widely-used general-purpose representations, such as single embedding and (contextualized) word embeddings.
%in the similarity between text.
%, for various unsupervised semantic tasks.

%We can call our method 
%Sent2Topics or Phrase2Topics



%we will explore how the codebook embeddings can be used to improve the performances of various unsupervised semantic tasks. 
%Due to the difficulty of evaluating the topics conditioned on the input sequence using the classic metrics for global topic modeling, we show that the codebook embeddings can be used to improve the performances of various unsupervised semantic tasks, which indirectly measures the quality of the generated topics.

%emphasize that we can make neural model more interpretable
%1. emphasize that the current benchmark is usually based on predicting similarity which could be done well in the traditional model
%2. put the randomly selected first 100 validation examples (in domain and out of domain) into supplementary material

\subsection{Experiment Setup}
\label{sec:exp_setup}
Our models only require the raw corpus and sentence/phrase boundaries, so we will only compare them with other unsupervised alternatives that do not require any manual labels or multi-lingual resources such as PPDB~\citep{pavlick2015ppdb}. To simplify the comparison, we also omit the comparison with the methods using character-level information such as fastText~\citep{bojanowski2017enriching} or bigram information such as Sent2Vec~\citep{pagliardini2018unsupervised}.

%do not need resources such as PPDB~\citep{pavlick2015ppdb} or other multi-lingual resources, so our models are compared with the baselines that only use the raw text and sentence/phrase boundaries. 

It is hard to make a fair comparison with BERT~\citep{BERT}. Its masked language modeling loss is designed for downstream supervised tasks and 
%BERT is designed as a pre-trained language model for supervised tasks, so it 
preserves more syntax information which might be distractive in unsupervised semantic applications. Furthermore, BERT uses word piece tokenization while other models use word tokenization. Nevertheless, we still present the performances of the BERT Base model as a reference even though it is trained using more parameters, larger embedding size, larger corpus, and more computational resources compared with our models. Since we focus on unsupervised setting, we directly use the final hidden states of the BERT models without supervised fine-tuning in most of the comparisons. One exception is that we also report the performance of sentence-BERT~\citep{reimers2019sentence} in a low-resource setting.
%trained on 100 labels to justify our unsupervised setting.
%are not fine-tuned using label data ex
%is trained on a masked language modeling loss and

%its unsupervised performances based on cosine similarity as a reference.
%We report the performance of the BERT base model while 
%to alleviate the out-of-vocabulary problem. 


%parse tree,

Our model is trained on English Wikipedia 2016 while the stop words are removed from the set of co-occurring words. In the phrase experiments, we only consider noun phrases, and their boundaries are extracted by applying simple regular expression rules to POS tags before training. We use the cased version (840B) of GloVe embedding~\citep{glove} as the pre-trained word embedding space for our sentence representation and use the uncased version (42B) for phrase representation.\footnote{\footnotesize\url{nlp.stanford.edu/projects/glove/}} To control the effect of embedding size, we set the hidden state size in our transformers as the GloVe embedding size (300).

Limited by computational resources, we train all the models using one GPU (e.g., NVIDIA 1080 Ti) within a week. Because of the relatively small model size, we find that our models underfit the data after a week (i.e., the training loss is very close to the validation loss). 

%given an input phrase or an unseen input sentence
\begin{table}[t!]

%are closest to the codebook embedding (in terms of cosine distances) and their corresponding cosine similarities.}
%the nearest three neighbors in a GloVe embedding space and their cosine similarities to the embedding.}
\scalebox{0.85}{
\begin{tabular}{|p{9.3cm}|}
\Xhline{5\arrayrulewidth}
\textbf{Input Phrase}: civil order \lessgreat{eos} \\ \Xhline{5\arrayrulewidth}
\textbf{Output Embedding (K = 1)}: \\ 
e1 \: | \space government 0.817 civil 0.762 citizens 0.748 \\ \hline
\textbf{Output Embeddings (K = 3)}: \\ 
e1 \: | \space initiatives 0.736 organizations 0.725 efforts 0.725 \\
e2 \: | \space army 0.815 troops 0.804 soldiers 0.786 \\
e3 \: | \space court 0.758 federal 0.757 judicial 0.736 \\ \hline
\multicolumn{1}{c}{}\\ \Xhline{5\arrayrulewidth}
\textbf{Input Sentence}: SMS messages are used in some countries as reminders of hospital appointments . \lessgreat{eos} \\ \Xhline{5\arrayrulewidth}
\textbf{Output Embedding (K = 1)}: \\  
 e1 \: | \space information 0.702, use 0.701, specific 0.700 \\ \hline
\textbf{Output Embeddings (K = 3)}: \\  
 e1 \: | \space can 0.769, possible 0.767, specific 0.767 \\
 e2 \: | \space hospital 0.857, medical 0.780, hospitals 0.739 \\
 e3 \: | \space SMS 0.791, Mobile 0.635, Messaging 0.631 \\ \hline
 \textbf{Output Embeddings (K = 10)}: \\
 e1 \: | \space can 0.854, should 0.834, either 0.821 \\
 e2 \: | \space hospital 0.886, medical 0.771, hospitals 0.745 \\
 e3 \: | \space services 0.768, service 0.749, web 0.722 \\
 e4 \: | \space  SMS 0.891, sms 0.745, messaging 0.686 \\
 e5 \: | \space messages 0.891, message 0.801, emails 0.679 \\
 e6 \: | \space systems 0.728, technologies 0.725, integrated 0.723 \\
 e7 \: | \space appointments 0.791, appointment 0.735, duties 0.613 \\
 e8 \: | \space confirmation 0.590, request 0.568, receipt 0.563 \\ 
 e9 \: | \space countries 0.855, nations 0.737, Europe 0.732 \\
 e10 | \space Implementation 0.613, Application 0.610, Programs 0.603\\ \hline 
 %\quad \;\: | \space Programs 0.603 \\ \hline 
\end{tabular}
}
\centering
\caption{Examples of the codebook embeddings predicted by our models with different $K$. The embedding in each row is visualized by the three words whose GloVe embeddings have the highest cosine similarities (also presented) with the codebook embedding.}
\label{tb:visual_example}
\end{table}
%The vectors are sorted by the predicted importance

\subsection{Qualitative Evaluation}
The cluster centers predicted by our model are visualized in Table~\ref{tb:visual_example} (as using \emph{girl} and \emph{lady} to visualize the red cluster center in Figure~\ref{fig:architecture}). Some randomly chosen examples are also visualized in \refappexample.

The centers summarize the input sequence well and more codebook embeddings capture more fine-grained semantic facets of a phrase or a sentence. Furthermore, the embeddings capture the compositional meaning of words. For example, each word in the phrase \emph{civil order} does not mean \emph{initiatives}, \emph{army}, or \emph{court}, which are facets of the whole phrase. When the input is a sentence, we can see that the output embeddings are sometimes close to the embeddings of words in the input sentence, which explains why attending the contextualized word embeddings in our decoder 
%the attention link between our encoder and decoder 
could improve the quality of the output embeddings.

%For phrases, all datasets we use lowercase the words
%For sentence, all datasets we use do not lowercase the words.
%820B
%42B


\subsection{Unsupervised Sentence Similarity}
\label{sec:STS}
We propose two ways to evaluate the multi-facet embeddings using sentence similarity tasks. 

\textbf{First way}: Since similar sentences should have similar word distribution in nearby sentences and thus similar codebook embeddings, the codebook embeddings of a query sentence $\bm{\widehat{F}_u(S^1_q)}$ should be able to well reconstruct the codebook embeddings of its similar sentence $\bm{\widehat{F}_u(S^2_q)}$. We compute the reconstruction error of both directions and add them as a symmetric distance \textbf{SC}:

%For our model, we evaluate two scoring functions that measure phrase similarity. 
%The similar phrases should have similar multi-facet embeddings, so we compute the reconstruction error from the set of normalized codebook embeddings of one phrase $S^1_q$ to the embeddings of the other phrase $S^2_q$, vice versa, and add them together to become a symmetric distance \textbf{SC}:

\vspace{-3mm}
\small
\begin{align}
 SC(S^1_q, S^2_q) & = Er(\bm{\widehat{F}_u(S^1_q)}, \bm{\widehat{F}_u(S^2_q))}  \nonumber \\
 & + Er(\bm{\widehat{F}_u(S^2_q)}, \bm{\widehat{F}_u(S^1_q)}), 
\label{eq:sc}
\end{align}
\normalsize
where $\bm{\widehat{F}_u(S_q)} = [ \frac{\underline{\vc}^q_k}{||\underline{\vc}^q_k||}  ]_{k=1...K}$ is a matrix of normalized codebook embeddings and $Er$ function is defined in~\eqref{eq:er}. We use the negative distance to represent similarity. 
%When ranking for retrieving similar phrases, 

\textbf{Second way}: 
One of the main challenges in unsupervised sentence similarity tasks is that we do not know 
%the lack of knowledge that 
which words are more important in each sentence. 
Intuitively, if one word in a query sentence is more important, the chance of observing related/similar words in the nearby sentences should be higher.
%the words in the nearby sentences should be more likely to be related to that word. 
Thus, we should pay more attention to the words in a sentence that have higher cosine similarity with its multi-facet embeddings, a summary of the co-occurring word distribution. Specifically, our importance/attention weighting for all the words in the query sentence $S_q$ is defined by

\vspace{-3mm}
\small
\begin{align}
\bm{\underline{a}_q} &= \max(0, \bm{W(S_q)}^T \bm{\widehat{F}_u(S_q)} ) \; \underline{\textbf{1}}, 
\label{eq:attention}
\end{align}
\normalsize
where $\underline{\textbf{1}}$ is an all-one vector. We show that the attention vector (denoted as \textbf{Our a} in Table~\ref{tb:STS}) could be combined with various scoring functions and boost their performances. 
%To justify the proposed NNSC loss, 
As a baseline, we also report the performance of the attention weights derived from the k-means loss rather than NNSC loss and call it \textbf{Our a (k-means)}.

%Since our multi-facet embeddings are in the same space of word embeddings, we can use the multi-facet embeddings to estimate the word importance (in terms of predicting possible co-occurring words beside the sentence). 
%To compute the importance of a word in the sentence, we first compute the cosine similarities between the word and all predicted codebook embeddings, truncate the negative similarity to 0, and sum all similarities.
%Specifically, our simple importance/attention weighting for all the words in the query sentence $S_q$ is defined by
%In response, we propose an attention-based weighting method that emphasizes the words in the sentence that are closer to the codebook embeddings. Specifically, the weights vector is computed by
%way to estimating the weights of each word

%\normalsize
%\underline{b}_q = A_q^T \underline{\textbf{1}} , A_q = \max(0, \widehat{F}_u(S_q)^TW(S_q) ) \\
%(S_q) &= W(S_q)\underline{a}_q, \nonumber \\

%\begin{table*}[t!]
\begin{figure*}[t!]
\scalebox{0.75}{
\begin{tabular}{|c|l|l|}
\hline
Sentences & \multicolumn{1}{|c|}{\colorbox{c79}{A} \colorbox{c27}{man} \colorbox{c50}{is} \colorbox{c21}{lifting} \colorbox{c23}{weights} \colorbox{c58}{in} \colorbox{c49}{a} \colorbox{c45}{garage} \colorbox{c63}{.}} & \multicolumn{1}{|c|}{\colorbox{c83}{A} \colorbox{c41}{man} \colorbox{c56}{is} \colorbox{c07}{lifting} \colorbox{c10}{weights} \colorbox{c66}{.}}   \\ \hline
& e1 \: | \space  can 0.872, even 0.851, should 0.850 & e1 \: | \space can 0.865, either 0.843, should 0.841 \\
& e2 \: | \space  front 0.762, bottom 0.742, down 0.714 & e2 \: | \space front 0.758, bottom 0.758, sides 0.691  \\
& e3 \: | \space  lifting 0.866, lift 0.663, Lifting 0.621 & e3 \: | \space lifting 0.847, lift 0.635, Lifting 0.610   \\
& e4 \: | \space  garage 0.876, garages 0.715, basement 0.707 & e4 \: | \space lifting 0.837, lift 0.652, weights 0.629   \\
Output& e5 \: | \space  decreasing 0.677, decreases 0.655, negligible 0.649 & e5 \: | \space decreasing 0.709, decreases 0.685, increases 0.682  \\
Embeddings& e6 \: | \space  weights 0.883, Weights 0.678, weight 0.665 & e6 \: | \space weights 0.864, weight 0.700, Weights 0.646  \\
& e7 \: | \space  cylindrical 0.700, plurality 0.675, axial 0.674 & e7 \: | \space annular 0.738, cylindrical 0.725, circumferential 0.701  \\
& e8 \: | \space  configurations 0.620, incorporating 0.610, utilizing 0.605 & e8 \: | \space methods 0.612, configurations 0.610, graphical 0.598  \\
& e9 \: | \space  man 0.872, woman 0.682, men 0.672 & e9 \: | \space sweating 0.498, cardiovascular 0.494, dehydration 0.485  \\
& e10 | \space  man 0.825, men 0.671, woman 0.653 & e10 | \space man 0.888, woman 0.690, men 0.676 \\ \hline
\end{tabular}
}
\centering
\caption{Comparison of our attention weights and the output embeddings between two similar sentences from STSB. A darker red indicates a larger attention value in \eqref{eq:attention} and the output embeddings are visualized using the same way in Table~\ref{tb:visual_example}.
}
\label{tb:good_topics_STS_main_paper}
%\end{table*}
\end{figure*}


\begin{table}[t!]
\scalebox{0.84}{
\begin{tabular}{|cc|cc|cc|}
\hline
\multicolumn{2}{|c|}{Method} & \multicolumn{2}{|c|}{Dev} & \multicolumn{2}{|c|}{Test} \\ \hline
\multicolumn{1}{|c|}{Score} & Model & All & Low & All & Low   \\ \hline
%ST & \multicolumn{1}{|c|}{Cos} & 34.6 & 40.6 & 24.5 & 17.8 \\ \hline
\multicolumn{1}{|c|}{Cosine} & Skip-thought & 43.2 & 28.1 & 30.4 & 21.2 \\ \hline
\multicolumn{1}{|c|}{CLS} & \multirow{2}{*}{BERT} & 9.6	& -0.4 & 4.1 & 0.2 \\
\multicolumn{1}{|c|}{Avg} &  &62.3 & 42.1 & 51.2 & 39.1 \\ \hline
\multirow{2}{*}{SC} & \multicolumn{1}{|c|}{Our c K1} & 55.7 & 43.7 & 47.6 & 45.4 \\
 & \multicolumn{1}{|c|}{Our c K10} & 63.0 & 51.8 & 52.6 & 47.8 \\ \hline
\multirow{3}{*}{WMD} & \multicolumn{1}{|c|}{GloVe} & 58.8 & 35.3 & 40.9 & 25.4 \\
 & \multicolumn{1}{|c|}{Our a K1} & 63.1 & 43.3 & 47.5 & 34.8 \\
 & \multicolumn{1}{|c|}{Our a K10} & 66.7 & 47.4 & 52.6 & 39.8 \\ \hline
\multirow{3}{*}{Prob\_WMD} & \multicolumn{1}{|c|}{GloVe} & 75.1 & 59.6 &	63.1 &	52.5 \\
 & \multicolumn{1}{|c|}{Our a K1} & 74.4 &	60.8 &	62.9 &	54.4 \\
 & \multicolumn{1}{|c|}{Our a K10} & \textbf{76.2} & \textbf{62.6} & \textbf{66.1} & 58.1 \\ \hline
\multirow{3}{*}{Avg} & \multicolumn{1}{|c|}{GloVe} & 51.7	& 32.8 & 36.6 & 30.9 \\
 & \multicolumn{1}{|c|}{Our a K1} & 54.5 & 40.2 & 44.1 & 40.6 \\
 & \multicolumn{1}{|c|}{Our a K10} & 61.7 & 47.1 & 50.0 & 46.5 \\ \hline
\multirow{3}{*}{Prob\_avg} & \multicolumn{1}{|c|}{GloVe} & 70.7 & 56.6 & 59.2	& 54.8 \\
& \multicolumn{1}{|c|}{Our a K1} & 68.5 & 56.0 & 58.1 & 55.2  \\
 & \multicolumn{1}{|c|}{Our a K10} & 72.0 & 60.5 & 61.4 & \textbf{59.3} \\ \hline
\multirow{4}{*}{SIF$\dagger$} & \multicolumn{1}{|c|}{GloVe} & 75.1 & 65.7 & 63.2 & 58.1 \\
 & \multicolumn{1}{|c|}{Our a K1} & 72.5 & 64.0 & 61.7 & 58.5 \\
 & \multicolumn{1}{|c|}{Our a K10} & \textbf{75.2} & \textbf{67.6} & \textbf{64.6} & \textbf{62.2} \\ 
  & \multicolumn{1}{|c|}{Our a (k-means) K10} & 71.5&	62.3&	61.5&	57.2 \\ 
 \hline \hline
\multicolumn{2}{|c|}{sentence-BERT (100 pairs)*} &71.2&55.5&64.5&58.2 \\ \hline

% \multicolumn{2}{|c|}{Method} & \multicolumn{2}{|c|}{Dev} & \multicolumn{2}{|c|}{Test} \\ \hline
% \multicolumn{1}{|c|}{Model} & Score & All & Low & All & Low   \\ \hline
% %ST & \multicolumn{1}{|c|}{Cos} & 34.6 & 40.6 & 24.5 & 17.8 \\ \hline

% \multirow{2}{*}{BERT} & \multicolumn{1}{|c|}{CLS} & 9.6	& -0.4 & 4.1 & 0.2 \\
%  & \multicolumn{1}{|c|}{Avg} &62.3 & 42.1 & 51.2 & 39.1 \\ \hline
% \multirow{5}{*}{GloVe} & \multicolumn{1}{|c|}{WMD} & 58.8 & 35.3 & 40.9	& 25.4 \\
% & \multicolumn{1}{|c|}{Prob\_WMD} &  75.1 & 59.6 &	63.1 &	52.5 \\
%  & \multicolumn{1}{|c|}{Avg} & 51.6	& 32.8 & 36.6 & 30.9 \\
%  & \multicolumn{1}{|c|}{Prob\_avg} & 70.7 & 56.6 & 59.2	& 54.8 \\
%  & \multicolumn{1}{|c|}{SIF$\dagger$} & 75.1 & 65.7 & 63.2 & 58.1 \\ \hline
%  & \multicolumn{1}{|c|}{SC} & 55.7 & 43.7 & 47.6 & 45.4 \\
%  & \multicolumn{1}{|c|}{Prob\_WMD} &74.4 &	60.8 &	62.9 &	54.4  \\
% Ours & \multicolumn{1}{|c|}{Avg} & 54.5 & 40.2 & 44.1 & 40.6 \\
% K=1 & \multicolumn{1}{|c|}{Prob\_avg} & 68.5 & 56.0 & 58.1 & 55.2 \\
%  & \multicolumn{1}{|c|}{SIF$\dagger$} & 72.5 & 64.0 & 61.7 & 58.5 \\ \hline
%  & \multicolumn{1}{|c|}{SC} & 63.0 & 51.8 &  52.6 & 47.8 \\
%  & \multicolumn{1}{|c|}{Prob\_WMD} & \textbf{76.2} & \textbf{62.6} & \textbf{66.1} & 58.1 \\
% Ours & \multicolumn{1}{|c|}{Avg} & 61.7 & 47.1 & 50.0 & 46.5 \\
% K=10 & \multicolumn{1}{|c|}{Prob\_avg} & 72.0 & 60.5 & 61.4 & \textbf{59.3} \\
%  & \multicolumn{1}{|c|}{SIF$\dagger$} & \textbf{75.2} & \textbf{67.6} & \textbf{64.6} & \textbf{62.2} \\ \hline
\end{tabular}
}
\centering
\caption{Pearson correlation (\%) in the development and test sets in the STS benchmark. The performances of all sentence pairs are indicated as All. Low means the performances on the half of sentence pairs with lower similarity (i.e., STSB Low). Our c means our codebook embeddings and Our a means our attention vectors. * indicates a supervised method. $\dagger$ indicates the methods which use training distribution to approximate testing distribution. The best score with and without $\dagger$ are highlighted.}
\label{tb:STS}
\end{table}



\textbf{Setup}: 
STS benchmark~\citep{sts} is a widely used sentence similarity task. We compare the correlations between the predicted semantic similarity and the manually labeled similarity. We report Pearson correlation coefficient, which is strongly correlated with Spearman correlation in all our experiments.
%Each model predicts a semantic similarity score between each sentence pair, and the scores are compared with average similarity annotations using the Pearson correlation coefficient. 
Intuitively, when two sentences are less similar to each other, humans tend to judge the similarity based on how similar their facets are. Thus, we also compare the performances on the lower half of the datasets where their ground truth similarities are less than the median similarity in the dataset, and we call this benchmark STSB Low.
%similarity score
%We compare all the results in the development set and test set in Table~\ref{tb:STS}.

A simple but effective way to measure sentence similarity is to compute the cosine similarity between the average (contextualized) word embedding~\citep{sim_sum_baseline}.
%(contextualized) word embedding
%compose the (contextualized) word embedding to sentence embedding is to 
%compute cosine similarity between the average word embedding~\citep{sim_sum_baseline}. 
The scoring function is labeled as \textbf{Avg}. %In addition to \textbf{Avg},
Besides, we test the sentence embedding from BERT and from skip-thought~\citep{kiros2015skip} (denoted as \textbf{CLS} and \textbf{Skip-thought Cosine}, respectively). 

In order to deemphasize the syntax parts of the sentences, \citet{sif} propose to weight the word $w$ in each sentence according to $\frac{\alpha}{\alpha + p(w)}$, where $\alpha$ is a constant and $p(w)$ is the probability of seeing the word $w$ in the corpus. Following its recommendation, we set $\alpha$ to be $10^{-4}$ in this paper. After the weighting, we remove the first principal component of all the sentence embeddings in the training data as suggested by \citet{sif} and denote the method as \textbf{SIF}.
%adopt the post-processing method from \citet{sif} to remove the first principal component that is estimated using the training distribution and denote the method as \textbf{SIF}. 
The post-processing requires an estimation of testing embedding distribution, which is not desired in some applications, so we also report the performance before removing the principal component, which is called~\textbf{Prob\_avg}.  
%~\citep{singh2018context}

We also test word mover's distance (\textbf{WMD}) \citep{kusner2015word}, which explicitly matches every word in a pair of sentences. As we do in \textbf{Prob\_avg}, we apply $\frac{\alpha}{\alpha + p(w)}$ to \textbf{WMD} to down-weight the importance of functional words, and call this scoring function as~\textbf{Prob\_WMD}. When using \textbf{Our a}, we multiple our attention vector with the weights of every word (e.g., $\frac{\alpha}{\alpha + p(w)}$ for \textbf{Prob\_avg} and \textbf{Prob\_WMD}).

To motivate the unsupervised setting, we present the performance of sentence-BERT \citep{reimers2019sentence} that are trained by 100 sentence pairs. We randomly sample the sentence pairs from a data source that is not included in STSB (e.g., headlines in STS 2014), and report the testing performance averaged across all the sources from STS 2012 to 2016.
%The sentence pairs are randomly sampled
%a supervised model, under a low resource setting. We train sentence-BERT using randomly sampled 100 sentence pairs 
%from a data source (e.g., headlines in STS 2014), and report its testing performance averaged across all data sources from STS 2012 to 2016 that are not included in STSB . 
More details are included in \refappsentsim.




\textbf{Results}: 
In Figure~\ref{tb:good_topics_STS_main_paper}, we first visualize our attention weights in \eqref{eq:attention} and our output codebook embeddings for a pair of similar sentences from STSB to intuitively explain why modeling co-occurring distribution could improve the similarity measurement. 

Many similar sentences might use different word choices or using extra words to describe details, but their possible nearby words are often similar. For example, appending \emph{in the garage} to \emph{A man is lifting weights} does not significantly change the facets of the sentences and thus the word \emph{garage} receives relatively a lower attention weight. This makes its similarity measurement from our methods, \textbf{Our c} and \textbf{Our a}, closer to the human judgment than other baselines.
%the nearby words are less likely to be related to the detail. 



%The attention weights are visualized using red background. If one word is more likely to be similar to the words in the nearby sentences, it will get more attention and thus highlighted using darker red.

%This is because although the sentences using different word choices or using extra words to describe the details, the distribution of possible words in the nearby sentences is similar.
%appending "in the garage" after "A man is lifting weights" does not significantly change the existing aspects of the sentences.


%duplicate cluster
%more motivative examples could be seen in the appendix

In Table~\ref{tb:STS}, \textbf{Our c SC}, which matches between two sets of facets, outperforms \textbf{WMD}, which matches between two sets of words in the sentence, and also outperforms \textbf{BERT Avg}, especially in STSB Low. The significantly worse performances from \textbf{Skip-thought Cosine} justify our choice of ignoring the order in the co-occurring words.

All the scores in \textbf{Our * K10} are significantly better than \textbf{Our * K1}, which demonstrates the co-occurring word distribution is hard to be modeled well using a single embedding. 
%benefits of multi-mode representation. 
Multiplying the proposed attention weighting consistently boosts the performance in all the scoring functions especially in STSB Low and without relying on the generalization assumption of the training distribution. Finally, using k-means loss, \textbf{Our a (k-means) K10}, significantly degrades the performance compared to \textbf{Our a K10}, which justify the proposed NNSC loss. In \refappsentsim, our methods are compared with more baselines using more datasets to test the effectiveness of multi-facet embeddings and our design choices more comprehensively.

%from (weighted) averaging-based methods especially in STSB Low 

%In addition to \textbf{BERT CLS}, \textbf{BERT Avg}, and \textbf{GloVe Avg}, we compare our method with  

%The importance weighting is multiplied with the original weighting vectors on \textbf{GloVe Avg} (uniform weight), \textbf{GloVe Prob\_avg}, and \textbf{GloVe SIF} to generate the results of \textbf{Our Avg}, \textbf{Our Prob\_avg}, and \textbf{Our SIF}, respectively. 

%The strong performance of (weighted) average embedding ~\citep{sim_sum_baseline, sif} suggests that we should consider the embeddings of words in the sentence in addition to the sentence embedding(s) when measuring the sentence similarity. This is hard to be achieved in other sentence representation methods because their sentence embeddings and word embeddings are in different semantic spaces.

%you do not need to compare their topic distribution to measure.
%Since our model generate the topics relevant to each sentence, it is 



%estimated
%also recommend to remove the first principle component after the weighting. We 
%label 
%estimate the first principle component based on the training set in STS benchmark and 

%and two weighted  averaging baselines \textbf{GloVe Prob\_avg} and \textbf{SIF}~. 

%In some places (introduction or experiment), we should say 
%we also do pretty well in higher level in training dataset!
%The sentence in STS is usually short (e.g., average length in STS Dev is around 13)

%\cite{wic}


%Our model with bi-LSTM as the encoder and LSTM as the decoder is also compared.





%The experiments of hypernym detection and sentence similarity also demonstrate that keeping the sequence embedding and word embedding in the same space allows more ways of considering the words in the sequence and the relevant topics of the sequence together.


%Our model with bi-LSTM as the encoder and LSTM as the decoder is also compared.
%Ours

%biLSTM for encoder and LSTM for decoder
%STS performance -> doing well in validation implies doing well in downstream tasks as well? Compare with skip-thoughts. (Put the validation loss directly here)
%Validation loss is -0.1289 for LSTM
%-0.1439 for Transformer

%It also demonstrates that ignoring the word ordering information in the co-occurring words can help us to learn a compositional model which focuses more on the semantic side of information.


%as far as we know, our method is the first one which shows that deep neural network could also be used to improve averaging-based word embedding methods in a sentence similarity task without learning from any annotation.






%compare with embedding of words representation in the sentences (like BERT) in the sentence similarity task?
%If we perform much better than skip-thoughts using n_basis, we could hypothesize that dropping the word order help us to learn a better sentence similarity
%\cite{kiros2015skip}

% \begin{table}[t!]
% \centering
% \scalebox{0.82}{
% \begin{tabular}{|c|c|c|c|}
% \hline
% Method & ROUGE 1 & ROUGE 2 & ROUGE SU4 \\ \hline
% Rnd & 9.28 & 2.48 & 3.22 \\ \hline
% %norm_w_in_sent_freq_4$\dagger$ & 4.76 & 1.28 & 1.61 \\ \hline
% %sent_emb_cluster_word_freq_4 & 14.84 & 4.49 & 5.37 \\ \hline
% %sent_emb_dist_avg_freq_4 & 14.89 & 4.52 & 5.38 \\ \hline
% %W Cluster & 14.84 & 4.49 & 5.37 \\ \hline
% W Emb$\dagger$ & 4.76 & 1.28 & 1.61 \\ \hline
% Sent Emb & 14.89 & 4.52 & 5.38 \\ \hline
% Ours (K=3) & 13.71 & 3.64 & 4.83 \\ \hline
% Ours (K=10) & 15.44 & 4.61 & 5.68 \\ \hline
% Ours (K=50) & 16.39 & 5.33 & \textbf{6.22} \\ \hline
% Lead & \textbf{16.67} & \textbf{5.55} & 6.13 \\ \hline
% \end{tabular}
% }
% \caption{The F1 scores of different methods and different ROUGE versions. $\dagger$ indicates that the best scores observed when two sentences are selected. Other are the results when only one sentence is selected.}
% \label{tb:sum}
% \end{table}

\subsection{Unsupervised Extractive Summarization}
% in a Single Document
\label{sec:sum}
The classic representation of a sentence uses either a single embedding or the (contextualized) embeddings of all the words in the sentence. In this section, we would like to show that both options are not ideal for extracting a set of sentences as a document summary.
%unsupervised extractive summarization task.
%Extractive summarization could be viewed as picking a set of sentences which are most similar to the whole document.

Table~\ref{tb:visual_example} indicates that our multiple codebook embeddings of a sentence capture its different facets well, so we represent a document summary $S$ as the union of the multi-facet embeddings of the sentences in the summary $R(S) = \cup_{t=1}^T \{\widehat{F}_u(S_t)\}$, where $\{\widehat{F}_u(S_t)\}$ is the set of column vectors in the matrix $\bm{\widehat{F}_u(S_t)}$ of sentence $S_t$.

A good summary should cover multiple facets that well represent all topics/concepts in the document~\citep{kobayashi2015summarization}. The objective can be quantified as discovering a summary $S$ whose multiple embeddings $R(S)$ best reconstruct the distribution of normalized word embedding $\underline{\vw}$ in the document $D$~\citep{kobayashi2015summarization}. That is,

\vspace{-3mm}
\small
\begin{align}
\argmax_{S} \sum_{\underline{\vw} \in D} \frac{\alpha}{\alpha + p(w)} \max_{\underline{\vs} \in R(S)} \underline{\vw}^T\underline{\vs},
\label{eq:sum_select}
\end{align}
\normalsize
%where $\gamma_w$ is the importance of the word $w$, which is set as $\frac{\alpha}{\alpha + p(w)}$ as we did in Section~\ref{sec:STS}. 
where $\frac{\alpha}{\alpha + p(w)}$ is the weights of words we used in the sentence similarity experiments~\citep{sif}. %Section~\ref{sec:STS}. 
We greedily select sentences to optimize~\eqref{eq:sum_select} as in~\citet{kobayashi2015summarization}.
%\footnote{Notice that all the embedding vectors are normalized, so solving the objective function is the same as minimizing the kmeans loss $\argmin_{A} \sum_{\underline{\vw} \in D} \gamma_w \min_{\underline{\vs} \in C(A)} ||\underline{\vw}-\underline{\vs}||^2$}



%Our model can generate multiple codebook embeddings, which capture its different aspects as we see in Table~\ref{tb:visual_example}, to represent each sentence in the document.
%We can input each sentence in the document into our model and generate multiple codebook embeddings to represent different aspects of a sentence as we see in Table~\ref{tb:visual_example}. 
%Then, we can greedily select a set of sentences whose multi-facet embeddings best reconstruct the word distribution of the document using k-means loss~\citet{kobayashi2015summarization}, where the importance of each word in the document is weighted by~$\frac{\alpha}{\alpha + p(w)}$ as we did in Section~\ref{sec:STS}.

\begin{table}[t!]
\scalebox{0.9}{
\begin{tabular}{|c|c|ccc|}
\hline
Setting & Method & R-1 & R-2 & Len \\ \hline
\multirowcell{10}{Unsup, \\ No \\ Sent \\ Order} & Random & 28.1 & 8.0 & 68.7 \\ 
%norm_w_in_sent_freq_4$\dagger$ & 4.76 & 1.28 & 1.61 \\ \hline
%sent_emb_cluster_word_freq_4 & 14.84 & 4.49 & 5.37 \\ \hline
%sent_emb_dist_avg_freq_4 & 14.89 & 4.52 & 5.38 \\ \hline
%W Cluster & 14.84 & 4.49 & 5.37 \\ \hline
& Textgraph (tfidf)$\dagger$ & 33.2  & 11.8 & -  \\ 
& Textgraph (BERT)$\dagger$ & 30.8 & 9.6 &  - \\ 
& W Emb (GloVe) & 26.6 & 8.8 & 37.0 \\ 
& Sent Emb (GloVe) & 32.6 & 10.7 & 78.2 \\ 
& W Emb (BERT) & 31.3 & 11.2 & 45.0 \\ 
& Sent Emb (BERT) & 32.3  & 10.6 & 91.2 \\ 
& Our c (K=3) & 32.2 & 10.1 & 75.4 \\ 
& Our c (K=10) & 34.0 & 11.6 & 81.3 \\ 
& Our c (K=100) & \textbf{35.0} & \textbf{12.8} & 92.9 \\ \hline
\multirow{2}{*}{Unsup} & Lead-3 & 40.3 & 17.6 & 87.0  \\ 
& PACSUM (BERT)$\dagger$ & \textbf{40.7}  & \textbf{17.8}  & -  \\ \hline
Sup & RL* &  \textbf{41.7} & \textbf{19.5}  & - \\ \hline
\end{tabular}
}
\centering
\caption{The ROUGE F1 scores of different methods on CNN/Daily Mail dataset. The results with $\dagger$ are taken from~\citet{zheng2019sentence}. The results with * are taken from~\citet{celikyilmaz2018deep}. }
\label{tb:sum}
\end{table}

\textbf{Setup}:
We compare our multi-facet embeddings with other alternative ways of modeling the facets of sentences. A simple way is to compute the average word embedding as a single-facet sentence embedding.\footnote{Although \eqref{eq:sum_select} weights each word in the document, we find that the weighting $\frac{\alpha}{\alpha + p(w)}$ does not improve the sentence representation when averaging the word embeddings.}
%computing weighted average for the sentence embedding using  }
%The weighted average using $\frac{\alpha}{\alpha + p(w)}$ is not better here} 
This baseline is labeled as \textbf{Sent Emb}. Another way is to use the (contextualized) embedding of all the words in the sentences as different facets of the sentences. Since longer sentences have more words, we normalize the gain of the reconstruction similarity by the sentence length. The method is denoted as \textbf{W Emb}.
%\footnote{In contrast, the fixed number of codebook embeddings in our method avoids the problem}
We also test the baselines of selecting random sentences (\textbf{Rnd}) and first 3 sentences (\textbf{Lead-3}) in the document.

The results on the testing set of CNN/Daily Mail~\citep{cnn_dataset,cnn_dataset_split} are compared using F1 of ROUGE~\citep{rouge} in Table~\ref{tb:sum}. R-1, R-2, and Len mean ROUGE-1, ROUGE-2, and average summary length, respectively. All methods choose 3 sentences by following the setting in \citet{zheng2019sentence}. \emph{Unsup, No Sent Order} means the methods do not use the sentence order information in CNN/Daily Mail.

%or other English news corpora
In CNN/Daily Mail, the unsupervised methods which access sentence order information such as \textbf{Lead-3} have performances similar to supervised methods such as RL~\citep{celikyilmaz2018deep}. To evaluate the quality of unsupervised sentence embeddings, we focus on comparing the unsupervised methods which do not assume the first few sentences form a good summary.
%~\citep{bohn2018neural}

%a state-of-the-art approach in this evaluation
%the sentence order information is a very strong signal. For example, 

%We only report the best performance across the greedy selection procedure. All the best performances happen when only one sentence is selected except \textbf{W Emb}, which prefers to select shorter sentences. 

%~\citep{rouge,rouge-su4}
\textbf{Results}:
In Table~\ref{tb:sum}, predicting 100 clusters yields the best results. Notice that our method greatly alleviates the computational and sample efficiency challenges, which allows us to set cluster numbers $K$ to be a relatively large number.

The results highlight the limitation of classic representations. The single sentence embedding cannot capture its multiple facets. On the other hand, if a sentence is represented by the embeddings of its words, it is difficult to eliminate the bias of selecting longer or shorter sentences and a facet might be composed by multiple words (e.g., the input sentence in Table~\ref{tb:visual_example} describes a service, but there is not a single word in the sentence that means service).
%design an unsupervised scoring function which
%the individual words in each sentence might not correspond to the aspects of sentences well 



%each sentence has different number of words, which make the 

%representing a sentence as a single embedding () does not yield  does not perform well due to lack 
%and \textbf{W Emb}


%, and setting K = 100 gives us the best performance after selecting 3 sentences. This demonstrates that larger cluster numbers $K$ is desired in this application. 


%problem of word embedding




%We mainly compare the unsupervised methods which do not use sentence order information

%When using such information, the performance of unsupervised methods such as \textbf{Lead} could be very similar to supervised methods.

%sentence order is a very important information

% in the CNN/Daily Mail dataset. 



%(please refer to the supplementary materials for the comparison given the same number of words in the summary)
%Note that when representing each sentence using word embeddings (i.e., \textbf{W Emb (*)}), we found that optimizing normalized loss gain tends to select shorter sentences. This shows that the variable number of sentence embeddings makes the design of selection objective more complicated. %In contrast, our method is able to generate a fixed number of clusters for each sentence, which makes it more convenient to be applied to some downstream tasks such as summarization.

%the comparable performance to \textbf{Lead}, a very strong baseline in this dataset~\citep{bohn2018neural}, while being much better than other baselines. 


%show that output fixed number of clusters is helpful for summarization

%(select the sentences based on the word order is a strong baseline)



%one of the advantage of 


%By , .



%We compare 
%The previous unsupervised extractive summarization based on distributional embedding

% propose a greedy sentence selection procedure to minimize the distances between sentences embedding and all the words in the documents (i.e., selected  sentence can be viewed as cluster centers of all the words).


%sent_emb_cluster_word_freq_4, an improved version of \citep{sum_clustering}. We cluster words in documents and choose the sentences closest to each center

%similar to sent_emb_dist_avg_freq_4






%Modeling different aspects of a sentence is also useful in summarization.

%extractive summarization based on embedding %distribution:
%clustering based
%reconstruction based



 



%\citep{textrank}


%For each pair of topic, project them to the rest of topics. Then, compute the wasserstein distance between two topic distribution



%and BERT trains on a larger corpus and has a much larger model size and dimensions. 

%Use Amol’s code to visualize all sentences in one paragraph. It would be great to see some distribution slightly morph and sometimes completely jump to another area



\subsection{Unsupervised Phrase Similarity}
Recently, \citet{dubossarsky2018coming} discovered that the multiple embeddings of each word may not improve the performance in word similarity benchmarks even if they capture more senses or facets of polysemies.
%multiple sense embeddings of each word do not improve the performances in word similarity benchmarks. 
Since our method can improve the sentence similarity estimation, we want to see whether multi-facet embeddings could also help the phrase similarity estimation.

In addition to \textbf{SC} in \eqref{eq:sc}, we also compute the average of the contextualized word embeddings from our transformer encoder as the phrase embedding. We find that the cosine similarity between the two phrase embeddings is a good similarity estimation, and the method is labeled as \textbf{Ours Emb}. 

\begin{table}[t!]
\scalebox{0.87}{
\begin{tabular}{|cc|cc|c|c|}
\hline
\multicolumn{2}{|c|}{Method} & \multicolumn{2}{c|}{SemEval 2013} & Turney (5) & Turney (10)   \\ \hline %\cline{1-2}
\multicolumn{1}{|c|}{Model} & Score & AUC & F1 & Accuracy & Accuracy \\ \hline
\multirow{2}{*}{BERT} & \multicolumn{1}{|c|}{CLS} & 54.7 & 66.7 & 29.2 & 15.5  \\ 
 & \multicolumn{1}{|c|}{Avg} & 66.5 & 67.1 & 43.4 & 24.3  \\ \hline
GloVe & \multicolumn{1}{|c|}{Avg} & 79.5 & 73.7 & 25.9 & 12.9 \\ \hline
%\multicolumn{1}{|c|}{Word2Vec} & Avg & - & 65.5* & 39.6* & 19.8* & - & - & - \\ \hline
\multicolumn{1}{|c|}{FCT LM$\dagger$} & Emb & - & 67.2 & 42.6 & 27.6 \\ \hline
Ours& \multicolumn{1}{|c|}{SC} & 80.3 & 72.8 & 45.6 & 28.8   \\ 
(K=10) & \multicolumn{1}{|c|}{Emb} & 85.6 & 77.1 & 49.4 & 31.8  \\ \hline
Ours & \multicolumn{1}{|c|}{SC} & 81.1 & 72.7 & 45.3 & 28.4   \\ 
(K=1) & \multicolumn{1}{|c|}{Emb} & \textbf{87.8} & \textbf{78.6} & \textbf{50.3} & \textbf{32.5}  \\ \hline
\end{tabular}
}
\centering
\caption{Performance of phrase similarity tasks. Every model is trained on a lowercased corpus. In SemEval 2013, AUC (\%) is the area under the precision-recall curve of classifying similar phrase pairs. In Turney, we report the accuracy (\%) of predicting the correct similar phrase pair among 5 or 10 candidate pairs. The results with $\dagger$ are taken from~\citet{fct}. }
%$\dagger$The results are taken from~\citet{WikiSRS}.   }
\label{tb:phrase_sim}
\end{table}

\textbf{Setup}:
We evaluate our phrase similarity using SemEval 2013 task 5(a) English~\citep{semeval2013} and Turney 2012~\citep{turney2012}. The task of SemEval 2013 is to distinguish similar phrase pairs from dissimilar phrase pairs. In Turney (5), given each query bigram, each model predicts the most similar unigram among 5 candidates, and Turney (10) adds 5 more negative phrase pairs by pairing the reverse of the query bigram with the 5 unigrams. 

%are two standard benchmarks for evaluating ~\citep{fct, huang2017learning}
%We compare our performance with 5 baselines. \textbf{GloVe Avg}  computes the cosine similarity between two averaged word embeddings, which has been shown to be a strong baseline~\citep{bird-naacl2019}. \textbf{BERT CLS} and \textbf{BERT Avg} are the cosine similarities between CLS embeddings and between the averages of contextualized word embeddings from BERT~\citep{BERT}, respectively. \textbf{FCT LM Emb}~\citep{fct} learns the weights of linearly combining word embeddings based on several linguistic features.

\textbf{Results}:
The performances are presented in Table~\ref{tb:phrase_sim}. \textbf{Ours (K=1)} is usually slightly better than \textbf{Ours (K=10)}, and the result supports the finding of~\citet{dubossarsky2018coming}. We hypothesize that unlike sentences, most of the phrases have only one facet/sense, and thus can be modeled by a single embedding well. In \refapphyper, the hypernym detection results also support this hypothesis.
%in sentence entailment and 
%there are not many polysemous phrases

Even though being slightly worse, the performances of \textbf{Ours (K=10)} remain strong compared with baselines. This implies that the similarity performances are not sensitive to the number of clusters as long as sufficiently large K is used because the model is able to output multiple nearly duplicated codebook embeddings to represent one facet (e.g., using two centers to represent the facet related to \emph{company} in Figure~\ref{fig:first_page}). The flexibility alleviates the issues of selecting K in practice. Finally, the strong performances in Turney (10) verify that our encoder respects the word order when composing the input sequence.
%considers the word order when producing phrase embeddings. 

%that multi-mode embeddings may not improve the performance in word similarity benchmarks even if they capture more senses or aspects of polysemies. 

%Our models significantly outperform all baselines in the 4 datasets.
%, especially by 21.1 AUC points in SemEval 2013 compared with \textbf{BERT Avg} and by 24.4 points in Turney (5) compared with \textbf{GloVe Avg}. 
%The results indicate the effectiveness of non-linearly composing word embeddings (unlike GloVe, Word2Vec, and FCT baselines) in order to predict the set of co-occurring word embeddings (unlike the BERT baselines).







%Semeval 2013 task 5(a) English~\citep{semeval2013} and Turney 2012~\citep{turney2012} are two standard benchmarks for evaluating phrase similarity~\citep{fct, huang2017learning}. In the test set of Semeval 2013, there are 3907 similar phrase pair and 3907 dissimilar phrase pairs and the task is to identify the similar phrase. In the test set of Turney 2012, there are 1500 questions and each question presents one query bigram and 5 candidate unigram.\footnote{We follow the evaluation setup of previous work~\citep{fct, huang2017learning}, which ignores the negative candidates being contained in the target phrase, because the original setup~\citep{turney2012} is too difficult for unsupervised methods to get a meaningful score (e.g., the accuracy of averaging the GloVe vector is 0 in the original setting). }  Turney (5) is to identify the unigram which is most similar to the bigram, and Turney (10) add 5 more negative pairs by reversing the word order in the bigram. 

%If the similarity measurement provides

%AUC
%average precision of retrieving similar phrase pairs
%codebook


%Emb
%BERT CLS
%BERT Avg












%present both with and without stop words
%In phrase dataset, we also present the results of frequency weighting method

%we can also argue that n\_basis = 1 does not do well in the distributional semantic space.

%We purely exploit the co-occurrence distribution rather than relying frequency information. The frequency information is a very effective signal for some datasets, but it might also be misleading in other datasets~\citep{dive}

%compare with AL1 DIVE and SBOW in DIVE paper in HypeNet (highlight that they are slightly different)


==> AAAI 2021 NSD/introduction.tex <==
%3 minutes presentation to IBM is a good way
%Related work summary in my slides (organize them into a table)
%we should stick with the conditional clustering plan because I know the related work better
%or suffering from not enough samples points (clustering approach)



%Start from asking what we can learn from only co-occurrence data without any supervision? 
%or composing manual rules 
%such as scientific literature. 

%only co-occurrence statistics in
%(contextualized) 

Collecting manually labeled data is an expensive and tedious process for new or low-resource NLP applications. 
Many of these applications require the text similarity measurement based on the text representation learned from 
%models that learn the representation from 
the raw text without any supervision. 
Examples of the representation include word embedding like Word2Vec~\citep{word2vec} or GloVe~\citep{glove}, sentence embeddings like skip-thoughts~\citep{kiros2015skip}, contextualized word embedding like ELMo~\citep{ELMo} and BERT~\citep{BERT} without fine-tuning. 

The existing work often represents a word sequence (e.g., a sentence or a phrase) as a single embedding. However, when squeezing all the information into a single embedding (e.g., by averaging the word embeddings or using CLS embedding in BERT), the representation might lose some important information of different facets in the sequence.

%The existing work typically represents a word sequence (e.g., a sentence or a phrase) by either a single embedding or the embedding of all the words in the sequence. In some unsupervised semantic applications, both solutions are not ideal. When using all the word embeddings in a sequence, the embeddings might not reflect the compositional meaning (e.g., a \emph{hot dog} is a food). In a long sequence,  embeddings of many words could make similarity estimation inefficient~\cite{luan2020sparse} and some words might be redundant or not important. Moreover, the variable number of embeddings could make some unsupervised scoring functions biased toward longer or shorter sequences (as we will show in our summarization experiments). On the other hand, when squeezing all the information into a single embedding (e.g., by averaging the word embeddings or using CLS embedding in BERT), the representation might lose some important information of different facets in the sequence.

%  because some embeddings might be redundant
%Parts of the representation , and 
%Using many embeddings to represent a long sentence is not efficient in retrieval applications~\cite{luan2020sparse}. 


%squeeze very different aspects into
%embedding does not consider the multiple aspects in the sentence.

%summarization 
%create some biases toward choosing longer or shorter sentences.
%when the number of embeddings is not fixed, it might 

%unsupervised summarization task

\begin{figure}[t!]
\begin{center}
\includegraphics[width=1\linewidth]{figures/First_page_figure_simple_preprint.pdf}
\end{center}
\caption{The input phrase \emph{real property} is represented by $K=5$ cluster centers. The previous work discovers the multiple senses by 
clustering the embedding of observed co-occurring words.
Instead, our compositional model learns to predict the embeddings of cluster centers from the sequence of words in the input phrase so as to reconstruct the (unseen) co-occurring distribution well.}
\label{fig:first_page}
\end{figure}

%finding cluster centers that well compress the embedding of observed co-occurring words. 
%represents a sentence or a phrase


%These models use a single embedding to represent one word or one sentence, which fails to capture multiple senses of a word and multiple aspects of a sentence. Recently, language modeling approaches like ELMo~\citep{ELMo} and BERT~\citep{BERT} provide contextualized embedding for each word in a sentence/phrase, but the models do not cluster the contexts of a phrase into senses and do not cluster words in a sentence into aspects.

%without label data, 
%cannot answer what senses a phrase have in a corpus and which aspect each word belongs to in a sentence.

%but a word might have multiple senses and a sentence can involve multiple topics. 

%, and contextualized word embedding like ELMo~\citep{ELMo} and BERT~\citep{BERT}. Most of these models either use a single embedding to represent one sentence/phrase or provide (contextualized) embedding for each word in the sentence/phrase. 
%However, when a sentence/phrase is represented by a single embedding, it does not 

%However, a word or phrase might have multiple senses, and a sentence can involve multiple topics, which are hard to analyze based on a single embedding without supervision.

%This setting is particularly practical for the domains with low resources such as scientific literature.

%and can only provide symmetric similarity measurement when no annotation is available. 
%directly introduce multiple embedding approach to explain the benefits
 %representing a facet of the input word sequence. 

Inspired by the multi-sense word embeddings~\citep{lau2012word,NeelakantanSPM14, athiwaratkun2017multimodal, singh2020context}, we propose a multi-facet representation that characterizes a phrase or a sentence as a fixed number of embeddings, where each embedding is a clustering center of the words co-occurring with the input word sequence. 

In this work, a facet refers to a mode of the co-occurring word distribution, which might be multimodal. For example, the multi-facet representation of \emph{real property} is illustrated in Figure~\ref{fig:first_page}. Real property can be observed in legal documents where it usually means real estate, while real property can also mean a true characteristic in philosophic discussions. The previous unsupervised multi-sense embeddings discover those senses by clustering the observed neighboring words (e.g., \emph{acquired}, \emph{save}, and \emph{tax}) and an important facet, a mode with high probability, could be represented by several close cluster centers. Notice that the approaches need to solve a distinct local clustering problem for each phrase in contrast with the topic modeling like LDA~\citep{blei2003latent}, which clusters all the words in the corpus into a global set of topics. 

%To address the issues, we extend the multi-sense word embedding methods to 


%word sense induction methods ~\citep{lau2012word} and recent multi-mode word embeddings~\citep{NeelakantanSPM14, athiwaratkun2017multimodal, singh2018context} represent each target word as multiple points or regions in a distributional semantic space by (explicitly or implicitly) clustering all the words appearing beside the target word. 






%,  while topic modeling 

%finds a single set of clusters by clustering all the words in the corpus.
%and each of clustering problem is solved based on only the words that co-occur with the target word.
%model multiple semantic aspects or senses of a target word


%Topic modeling solves only a single global clustering problem on all the words in the corpus, while multi-mode word embeddings solve a local clustering problem for only the co-occurring words of every target word in the vocabulary.

% represent each word as multiple points or regions by clustering  in order to . 
%pelevina2016making

%A natural extension of the clustering based methods is to

%As the length of input word sequence increases, 
In addition to a phrase, we can also cluster the nearby words of a sentence which appears frequently in the corpus. The cluster centers usually correspond to important aspects rather than senses (see an example in Figure~\ref{fig:architecture}) because a sentence usually has multiple aspects but only one sense. However, extending the clustering-based multi-sense word embeddings to long sequences such as sentences is difficult in practice due to two efficiency challenges. First, there are usually many more unique phrases and sentences in a corpus than there are words, while the number of parameters for clustering-based approaches is $O(|V| \times |K| \times |E|)$, where $|V|$ is the number of unique sequences, $|K|$ is the number of clusters, and $|E|$ is the embedding dimensions. Estimating and storing such a large number of parameters takes time and space. More importantly, much more unique sequences imply much fewer co-occurring words to be clustered for each sequence, especially for sentences. An effective model needs to overcome this sample efficiency challenge (i.e., sparseness in the co-occurring statistics), but clustering approaches often have too many parameters to learn the compositional meaning of each sequence without overfitting.

%the problem is not hopeless because

Nevertheless, the sentences (or phrases) sharing multiple words often lead to similar cluster centers, so we should be able to solve these local clustering problems using much fewer parameters to circumvent the challenges. 
To achieve the goal, we develop a novel Transformer-based neural encoder and decoder. As shown in Figure~\ref{fig:first_page}, instead of clustering co-occurring words beside an input sequence at test time as in previous approaches, we learn a mapping between the input sequence (i.e., phrases or sentences) and the corresponding cluster centers during training so that we can directly predict those cluster centers using a single forward pass of the neural network for an arbitrary unseen input sequence during testing.
%exploit redundancy in 
%many parameters could be compressed, and we use a neural network to do that.
%neural network in NLP can .

%When the model learns to predict the cluster centers during training, 
%To allow the neural network to generate the cluster centers in an arbitrary order, we use a non-negative and sparse coefficient matrix to dynamically match the sequence of predicted cluster centers and the observed set of co-occurring word embeddings during training. 
To train the neural model that predicts the clustering centers, we match the sequence of predicted cluster centers and the observed set of co-occurring word embeddings using a non-negative and sparse permutation matrix.
After the permutation matrix is estimated for each input sequence, the gradients are back-propagated to cluster centers (i.e.,  codebook embeddings) and to the weights of our neural model, which allows us to train the whole model end-to-end. 

% jointly and
%To show the effectiveness of multi-sense word embedding, the previous studies 

In the experiments, we evaluate whether the proposed multi-facet embeddings could improve the similarity measurement between two sentences, between a sentence and a document (i.e., extractive summarization), and between phrases. The results demonstrate multi-facet embeddings significantly outperforms the classic single embedding baseline when the input sequence is a sentence. 

We also demonstrate several advantages of the proposed multi-facet embeddings over the (contextualized) embeddings of all the words in a sequence. First, we discover that our model tends to use more embeddings to represent an important facet or important words. This tendency provides an unsupervised estimation of word importance, which improves various similarity measurements between a sentence pair. Second, our model outputs a fixed number of facets by compressing long sentences and extending short sentences. In unsupervised extractive summarization, this capability prevents the scoring function from biasing toward longer or shorter sentences. Finally, in the phrase similarity experiments, our methods capture the compositional meaning (e.g., a \emph{hot dog} is a food) of a word sequence well and the quality of our similarity estimation is not sensitive to the choice of \emph{K}, the number of our codebook embeddings.

%phrase
%When using all the word embeddings in a sequence, the embeddings might not reflect the compositional meaning (e.g., a \emph{hot dog} is a food). 

%attention
%some words might be redundant or not important. 
%Important facets
%K value, redundant cluster centers

%summarization
%Moreover, the variable number of embeddings could make some unsupervised scoring functions biased toward longer or shorter sequences (as we will show in our summarization experiments). 

%extend short sentence and compress long sentence if desired

%In experiments, we observe that multiple embeddings capture the facets of phrases and sentences well. and outperforms the classic single embedding representation and other strong unsupervised baselines in similarity and summarization tasks. On the other hand, a phrase usually have only one sense, so our multi-mode and single-mode phrase embeddings perform similarly well in similarity tasks, which supports the finding in \citet{dubossarsky2018coming}. 

%appears in one topic

\subsection{Main Contributions}
\label{sec:contributions}
%Our main contributions could be summarized as follows:
%We summarize our main contributions as follows:
%Our main contributions could be summarized as follows:
\setlist{nolistsep}
\begin{enumerate}
%~\reffgphrase, 
    %overcomes the sparsity challenges of co-occurring training signals by .
    \item As shown in Figure~\ref{fig:first_page},  
    we propose a novel framework that predicts the cluster centers of co-occurring word embeddings to overcomes the sparsity challenges in our self-supervised training signals.
    This allows us to extend the idea of clustering-based multi-sense embeddings to phrases or sentences.
    %, which limits the applicability of existing clustering-based multi-mode embeddings to phrases or sentences. 
    %to longer text sequence like phrases or sentences.
    %the limitations of existing clustering-based multi-mode embeddings
    %sparsity of training  challenges in the existing multi-mode embeddings. allow us to generate the multi-facet embedding for long sequence. Even for unseen ones.
    \item We propose a deep architecture that can effectively encode a sequence and decode a set of embeddings. We also propose non-negative sparse coding (NNSC) loss to train our neural encoder and decoder end-to-end.
    \item We demonstrate how the multi-facet embeddings could be used in unsupervised ways to improve the similarity between sentences/phrases, infer word importance in a sentence, extract important sentences in a document. In \refapphyper, we show that our model could provide asymmetric similarity measurement for hypernym detection. 
    %estimate the entailment relations between phrases.
    \item We conduct comprehensive experiments in the main paper and appendix to show that multi-facet embedding is consistently better than classic single-facet embedding for modeling the co-occurring word distribution of sentences, while multi-facet phrase embeddings do not yield a clear advantage against the single embedding baseline, which supports the finding in \citet{dubossarsky2018coming}.
%4. comprehensive experiments show when multi-facet embedding is better than classic single-facet embedding

\end{enumerate}
%In the supplementary materials, we also present the results of hypernymy detection to further support the observation.

%show that the multi-mode representation is shown to outperform the single-mode alternatives in sentence  representation 
%, especially as demonstrated in our extractive summarization experiment.
%the proposed model captures the compositional meanings of words in unsupervised phrase similarity tasks much better than averaging their (contextualized) word embeddings, strong baselines that are widely used in practice. In addition to similarity, our model can also measure asymmetric relations like hypernymy without any supervision. Furthermore, 

\begin{figure*}[t!]
\centering
\includegraphics[width=0.9\linewidth]{figures/architecture.pdf}
\caption{Our model for sentence representation. We represent each sentence as multiple codebook embeddings (i.e., cluster centers) predicted by our sequence to embeddings model. Our loss encourages the model to generate codebook embeddings whose linear combination can well reconstruct the embeddings of co-occurring words (e.g., \emph{music}), while not able to reconstruct the negatively sampled words (i.e., the co-occurring words from other sentences).} %to avoid predicting topics which are frequent but less informative. }
\label{fig:architecture}
\end{figure*}

%the specificity information of each phrase could also be preserved
%introduce non-negative sparse coding loss?

%

%, especially when the  when performing extractive summarization in a single document.

%when estimating semantic similarity between the sentences which are less similar in ground truth and

%estimate the reconstruction 
%The architecture could be viewed as a seq2seq model plus an end-to-end trainable coefficient matrix, which 

%Topics are a set
%we propose a set decoder module


%end to end 
%joint learning
%clustering centers

%conditioned on 
%Since our 
%the co-occurring words
%In order to 
%propose a novel neural decoder which

%At inference time, the set decoder directly predicts multiple cluster centers which compress the co-occurrence word distribution conditioned on the query phrase or sentence.

%In some places (introduction or experiment), we should say average embedding is still hard to beat in unsupervised setting

%\citep{singh2018context} (Context Mover's Distance)





%multi-modality representation
%Could infer entailment in a unsupervised way
%Learn how to compose arbitrary input features -> Overcome sparsity

%, we exploit the redundancy in these clustering problems by assuming that . 
%the concept of conditional clustering

%Several 
%region
%different aspects of a concept and

%The representation is hard to capture asymmetric relation entailment unless we have some supervised data

%clustering the co-occurrence
%word sense induction

%It is hard to use clustering approach to learn composition model for multiple words.


%too many different queries
%2 problems:
%sprase matrix problem
%Not time or memory efficient
%Storing lots of cluster centers take lots of space. If we want to do the clustering on the fly (especially for out of vocabulary words), clustering could be slow and hard to parallized.
%clustering for new words is expensive. 



%If we want to extend the multi-modal word representation to phrases or sentences, we will face two challenges
%time and memory efficiency issue
%sample efficiency issue



%Recent work~\citep{saphra2018understanding, tenney2018you} uses the training and testing data in various downstream tasks to interpret what semantic information and syntax properties are learned. However, we often do not have much annotated data in many applications. In these cases, understanding the learned embeddings of each phrase or sentence by checking their nearest neighbors in the embedding space seems to be the most popular option. The solution is unsatisfactory because it is hard to know a phrase consists of which senses, a sentence involves which topics, and two words or sentences are similar in which aspects.


%often cannot interpret what aspects 

%Rich semantic information and syntax properties in the embeddings are demonstrated to help various downstream tasks~\citep{saphra2018understanding, tenney2018you}. 



%\citep{ELMo,BERT}
%either single embedding to represent one sentence or one word (word2vec, seq2seq, language modeling) 

%complicated encoder
%The single embedding contains lots of information
%mixing semantic and syntax

%\citep{saphra2018understanding, tenney2018you}

%Two sentences, similar in which aspects?
%we can only measure similarity and it is hard to interpret the similarity
%BERT is not good for semantic task
%\citep{tenney2018you}


==> AAAI 2021 NSD/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> AAAI 2021 NSD/method.tex <==
%formalize and justify goal, 
%introduce two major components 

In this section, we first formalize our training setup and next describe our objective function and neural architecture. Our approach is visually summarized in Figure~\ref{fig:architecture}. 

%In this section, we first formalize our training setup in Section~\ref{sec:method_goal}. Our objective function and neural architecture will be described in Section~\ref{sec:method_loss} and Section~\ref{sec:method_neural}, respectively. Our approach is visually summarized in Figure~\ref{fig:architecture}. 
 %summarizes the approach.
 
 %The approach is summarized in . 
 %using an example sentence.

%Figure~\ref{fig:architecture} illustrates our goal and two major components in our proposed method.
%and explain our motivation 

\subsection{Self-supervision Signal}
\label{sec:method_goal}

We express $t$th sequence of words in the corpus as $I_t = w_{x_t} ... w_{y_t}$\lessgreat{eos}, where $x_t$ and $y_t$ are the start and end position of the input sequence, respectively, and \lessgreat{eos} is the end of sequence symbol.

We assume neighboring words beside each input phrase or sentence are related to some facets of the sequence, so given $I_t$ as input, our training signal is to reconstruct a set of co-occurring words, 
$N_t = \{w_{x_t-d^t_1}, ... w_{x_t-1}, w_{y_t+1}, ... w_{y_t+d^t_2}\}$.\footnote{The self-supervised signal is a generalization of the loss for prediction-based word embedding like Word2Vec~\citep{word2vec}. They are the same when the input sequence length $|I_t|$ is 1.} In our experiments, we train our multi-facet sentence embeddings by setting $N_t$ as the set of all words in the previous and the next sentence, and train multi-facet phrase embeddings by setting a fixed window size $d^t_1=d^t_2=5$.

%For phrase representation,  $d^t_1=d^t_2=5$ is a fixed window size. For sentence representation,  
%Notice that the training data for sentences and phrases are different, which means we need to train one model for phrase and one model for sentence if both representations are desired. 

%When arguing that we use the words in previous sentence and next sentence to represent this sentence, we say that the current sentence constrains the space of previous and next sentences. 
Since there are not many co-occurring words for a long sequence (none are observed for unseen testing sequences), the goal of our model is to predict the cluster centers of the words that could "possibly" occur beside the text sequence rather than the cluster centers of the actual occurring words in $N_t$ (e.g., the hidden co-occurring distribution instead of green and underlined words in Figure~\ref{fig:architecture}). The cluster centers of an unseen testing sequence are predictable because the model could learn from similar sequences and their co-occurring words in the training corpus.

%The prediction task of an unseen testing sequence can be learned well if the model observe many similar sequences and their co-occuring words in the training corpus.
%by observing co-occurring words of similar text sequences in our training corpus.

%Our models learn to predict the unseen 
%Although most of the possibly co-occurring words are not observed in the corpus, we can still learn to predict them by observing co-occurring words from similar text sequences in our training corpus.

To focus on the semantics rather than syntax, we view the co-occurring words as a set rather than a sequence as in skip-thoughts~\citep{kiros2015skip}. 
Notice that our model considers the word order information in the input sequence $I_t$, but ignores the order of the co-occurring words $N_t$.




%We assume that word distribution of previous sentence and next sentence will highly overlap with the word distribution of all possible ways of saying the current sentence and they won’t follow to a particular sequence of event with high probability (e.g., after we cook the dinner, we need the dinner).

%$|I_t| = y_t - x_t + 2$

%If we set the length of input sequence $|I_t|$ to be 1, the self-supervised signal is the same as prediction based word embedding like word2vec~\citep{word2vec}.

%generalize the word embedding methods


%Predicting sequence vs predicting sets. Focus more on the semantic rather than syntax \citep{kiros2015skip}

%Since we want to focus on the semantic, we disregard the orders in the co-occurring words.



\subsection{Non-negative Sparse Coding Loss}
\label{sec:method_loss}
%The prediction model 
%In this work, 
In a pre-trained word embedding space, we predict the cluster centers of the co-occurring word embeddings. The embeddings of co-occurring words $N_t$ are arranged into a matrix $\bm{W(N_t)} = [ \underline{\vw}^t_j]_{j=1...{|N_t|}}$ with size $|E| \times |N_t|$, where $|E|$ is the dimension of pre-trained word embedding, and each of its columns $\underline{\vw}^t_j$ is a normalized word embedding whose 2-norm is 1. The normalization makes the cosine distance between two words become half of their squared Euclidean distance. 

Similarly, we denote the predicted cluster centers $\underline{\vc}^t_k$ of the input sequence $I_t$ as a $|E| \times K$ matrix $\bm{F(I_t)} = [ \underline{\vc}^t_k]_{k=1...K}$, where $\bm{F}$ is our neural network model and $K$ is the number of clusters. 
We fix the number of clusters $K$ to simplify the design of our prediction model and the unsupervised scoring functions used in the downstream tasks. When the number of modes in the (multimodal) co-occurring distribution is smaller than $K$, the model can output multiple cluster centers to represent a mode (e.g., the \emph{music} facet in Figure~\ref{fig:architecture} is represented by two close cluster centers).
%That is, the hyperparameter $K$ means the maximal number of facets in our model and 
As a result, the performances in our downstream applications are not sensitive to the setting of $K$ when $K$ is larger than the number of facets in most input word sequences.
%The effect of different cluster numbers will be discussed in the experiments.

%denote the prediction model we want to find as $F$ and its 
The reconstruction loss of k-means clustering in the word embedding space %~\citep{singh2018context} 
can be written as $||\bm{F(I_t)}\bm{M} - \bm{W(N_t)}||^2 = \sum_j || (\sum_k \bm{M}_{k,j} \underline{\vc}^t_k)  - \underline{\vw}^t_j ||^2$, where $\bm{M}_{k,j}=1$ if the $j$th word belongs to the $k$ cluster and 0 otherwise. That is, $\bm{M}$ is a permutation matrix which matches the cluster centers and co-occurring words and allow the cluster centers to be predicted in an arbitrary order.
%the neural network to generate the centers in an arbitrary order. 

Non-negative sparse coding (NNSC)~\citep{hoyer2002non} relaxes the constraints by allowing the coefficient $\bm{M}_{k,j}$ to be a positive value but encouraging it to be 0. We adopt NNSC in this work because we observe that the neural network trained by NNSC loss generates more diverse topics than k-means loss does. We hypothesize that it is because the loss is smoother and easier to be optimized for a neural network. Using NNSC, we define our reconstruction error as

\vspace{-3mm}
\small
\begin{align}
& Er(\bm{F(I_t)},\bm{W(N_t)}) = ||\bm{F(I_t)}\bm{M^{O_t}} - \bm{W(N_t)}||^2 \nonumber \\ 
& s.t., \bm{M^{O_t}} = \argmin_{\bm{M}} ||\bm{F(I_t)}\bm{M} - \bm{W(N_t)}||^2 + \lambda || \bm{M} ||_1, \nonumber \\ 
& \forall k,j, \; 0 \leq \bm{M}_{k,j} \leq 1, 
\label{eq:er}
\end{align}
\normalsize
where $\lambda$ is a hyper-parameter controlling the sparsity of $\bm{M}$. We force the coefficient value $\bm{M}_{k,j}\leq 1$ to avoid the neural network learning to predict centers with small magnitudes which makes the optimal values of $\bm{M}_{k,j}$ large and unstable.


%stern2018blockwise

We adopt an alternating optimization strategy similar to the EM algorithm for k-means. At each iteration, our E-step estimates the permutation coefficient $\bm{M^{O_t}}$ after fixing our neural model, while our M-step treats $\bm{M^{O_t}}$ as constants to back-propagate the gradients of NNSC loss to our neural network.
%iterative training procedure 
A pseudo-code of our training procedure could be found in \refappalgo.
%Having multiple outputs and e
Estimating the permutation between the prediction and ground truth words is often computationally expensive~\citep{label_set}. Nevertheless, optimizing the proposed loss is efficient because 
for each training sequence $I_t$, $\bm{M^{O_t}}$ can be efficiently estimated using convex optimization (our implementation uses RMSprop~\citep{tieleman2012lecture}). Besides, we minimize the L2 distance, $||\bm{F(I_t)}\bm{M^{O_t}} - \bm{W(N_t)}||^2$, in a pre-trained embedding space as in~\citet{kumar2018mises,li2019efficient} rather than computing softmax. %Then, we treat $\bm{M^{O_t}}$ as constants and back-propagate the gradients to our neural network to achieve end-to-end training. 
%. After $\bm{M^{O_t}}$ is estimated

To prevent the neural network from predicting the same global topics regardless of the input, our loss function for $t$th sequence is defined as

\vspace{-3mm}
\footnotesize
\begin{align}
L_t(\bm{F}) = Er( \bm{F(I_t)} , \bm{W(N_t)} ) -   Er( \bm{F(I_t)} , \bm{W(N_{r_t}} )),
\label{eq:obj_func}
\end{align}
\normalsize
\noindent where $N_{r_t}$ is a set of co-occurring words of a randomly sampled sequence $I_{r_t}$. In our experiment, we use SGD to solve $\widehat{\bm{F}} = \argmin_{\bm{F}} \sum_t L_t(\bm{F})$. Our method could be viewed as a generalization of Word2Vec~\citep{word2vec} that can encode the compositional meaning of the words and decode multiple embeddings.

%word2vec~\citep{word2vec} did
%\begin{align}
%\widehat{F} = \argmin_F \sum_t Err( F(I_t)) , W(N_t)) )) \nonumber \\
%-   Err( F(I_t)) , W(N_{r_t})) ))
%\end{align}

%allow back-prop
%we solve F by SGD

%When talking about negative sampling
%say that our model is like skip gram, but have an encoder to model the composition and decode multiple embeddings rather than a single one.

%It is like word2vec~\citep{word2vec}

%In our implementation, we use RMSprop.

%Even though we predict a set of elements, our training
%we minimze the L2 
%Compared with other matching algorithm, optimizing $M^O$ is very efficient so that we do not need to 

%can be efficiently estimated by gradient descent based optimization. We use RMSprop and clamp the coefficient between 0 and 1 at each iteration in our experiments.

%we do not need to use computational expensive softmax loss 
%\citep{kumar2018mises} (Von Mises-Fisher Loss)


%we want our predicted cluster centers to reconstruct the distribution well. 
%encouraging $m^O_{k,j}$ to be 0 but allowing a positive value.



%\citep{hoyer2002non} (Non-negative Sparse Coding)
%Then, the reconstruction error could be written as $||F(I_t)M^O - W(N_t)||^2 = \sum_j || (\sum_k m^O_{k,j} \underline{c}^t_k)  - \underline{w}^t_j ||^2$


%with arbitrary order of word embedding in the matrix
%Kmeans, match perspective

%One of the main reasons that c
%We can use more cluster numbers to model the distribution better

%$|N_t|$ is the number of co-occurring words, 
%normalized to have norm 1 such that the Euclidean distance is the 2 * cosine distance.
%Our goal is to model 
%in a distributional semantic space, which is  .





%at once is
% intensive







%goal 
%use a fixed number of clusters K to well reconstruct













%$M^O$ with size $K \times |N_t|$








%\footnotesize
%\begin{align}

%\end{align}
%\normalsize

\subsection{Sequence to Embeddings}
\label{sec:method_neural}

Our neural network architecture is similar to Transformer-based sequence to sequence (seq2seq) model~\citep{vaswani2017attention}. We use the same encoder $TE(I_t)$, which transforms the input sequence into a contextualized embeddings

\vspace{-3mm}
\small
\begin{align}
[\underline{\ve}_{x_t} ... \underline{\ve}_{y_t} \underline{\ve}_{\text{\lessgreat{eos}}}] = TE( w_{x_t} ... w_{y_t}\text{\lessgreat{eos}} ),
\end{align}
\normalsize
where the goal of the encoder is to map the similar sentences, which are likely to have similar co-occurring word distribution, to similar contextualized embeddings.

Different from the typical seq2seq model~\citep{sutskever2014sequence, vaswani2017attention}, our decoder does not need to make discrete decisions because our outputs are a sequence of embeddings instead of words. This allows us to predict all the codebook embeddings in a single forward pass as in~\citet{lee2018set} without requiring an expensive softmax layer or auto-regressive decoding.\footnote{The decoder can also be viewed as another Transformer encoder which attends the output of the first encoder and models the dependency between predicted cluster centers.} 



%while still considering the dependency between output

To make different codebook embeddings capture different facets, we pass the embeddings of \lessgreat{eos}, $\underline{\ve}_{\text{\lessgreat{eos}}}$, to different linear layers $L_k$ before becoming the input of the decoder $TD$. The decoder allows the input embeddings to attend each other to model the dependency among the facets and attend the contextualized word embeddings from the encoder, $\underline{\ve}_{x_t} ... \underline{\ve}_{y_t}\underline{\ve}_{\text{\lessgreat{eos}}}$, to copy the embeddings of some keywords in the word sequence as our facet embeddings more easily.
%collect the information of some keywords in the word sequence.
%while still considering the dependency between output
Specifically, the codebook embeddings

%Similar to BERT, we treat the embedding of <eos> as the sentence representation. 

\vspace{-3mm}
\small
\begin{align}
\bm{F(I_t)} = TD(L_1(\underline{\ve}_{\text{\lessgreat{eos}}}) ... L_K(\underline{\ve}_{\text{\lessgreat{eos}}}), \underline{\ve}_{x_t} ... \underline{\ve}_{y_t}\underline{\ve}_{\text{\lessgreat{eos}}}).
\end{align}
\normalsize

We find that removing the attention on the $\underline{\ve}_{x_t} ... \underline{\ve}_{y_t}\underline{\ve}_{\text{\lessgreat{eos}}}$ significantly deteriorates our validation loss for sentence representation because there are often too many facets to be compressed into a single embedding. On the other hand, the encoder-decoder attention does not significantly change the performance of phrase representation, so we remove the connection (i.e., encoder and decoder have the same architecture) in models for phrase representation.
%and we remove the attention connection between encoder and decoder (i.e., encoder and decoder have the same architecture) when evaluating our phrase representation.
Notice that the framework is flexible. For example, we can encode the genre of the document containing the sentence if desired.
%Notice that the encoder and decoder can be can replaced with other architectures. 
%Besides transformers, we also try (bi-)LSTMs in our experiments. 
%This flexibility allows us to incorporate other input features (e.g., the author who writes the sentence).

%Different from typical seq2seq~\citep{sutskever2014sequence, vaswani2017attention}. 
%We do not make discrete decision
%Experiments show that transformer decoder can learn the dependency between the output codebook vectors well

%topics are continuous and have strong dependency between each other, so we cannot just do typical multi-label classification
%compared with multi-label classification, 

%encoder and decoder intuition
%Specifically, we learn an encoder to map similar sentences close to each other in a hidden embedding space and based on the encoded embeddings, we learn a decoder to predict a set of representative points which can well reconstruct the distribution of their co-occurring words in a pre-trained word embedding space. 

%The complexity of encoder and decoder. If the similar features  could have very different topics and we have enough observation of occurrence to do the clustering, the encoder should be complex. 
%The smoothness effect of decoder


%For instance, 
%use arbitrary encoder here to consider 
%Notice that encoder and decoder could be replaced by other neural network models. 

==> AAAI 2021 NSD/more_examples.tex <==
We visualize the predicted codebook embeddings and the attention weights computed using~\refeqatt~from 10 randomly selected sentences in our validation set (so most of them are unseen in our training corpus). 
%We upload a file called more\_example into the data category.


The first line of each example is always the preprocessed input sentence, where <unk> means an out-of-vocabulary placeholder. The attention weights are visualized using a red background. If one word is more likely to be similar to the words in the nearby sentences, it will get more attention and thus highlighted using a darker red color.

The format of visualized embeddings is similar to Table~\reftbvis%~\ref{tb:visual_example}
. Each row's embedding is visualized by the nearest five neighbors in a GloVe embedding space and their cosine similarities to the codebook embedding.

%The first section of file contains around the 100 examples where the unseen sentences come from the seen Wikipedia pages. The section starts with "Shuffled Validation Topics:". The second section contains another 100 examples where the unseen sentences come from the unseen Wikipedia pages. The section starts with "Validation Topics:". All the examples are randomly selected.


\colorbox{c87}{Other} \colorbox{c56}{immobilizing} \colorbox{c48}{devices} \colorbox{c57}{such} \colorbox{c60}{as} \colorbox{c62}{a} \colorbox{c73}{Kendrick} \colorbox{c100}{<unk>} \colorbox{c78}{Device} \colorbox{c58}{or} \colorbox{c62}{a} \colorbox{c53}{backboard} \colorbox{c53}{can} \colorbox{c58}{be} \colorbox{c60}{used} \colorbox{c62}{to} \colorbox{c46}{stabilize} \colorbox{c59}{the} \colorbox{c62}{remainder} \colorbox{c64}{of} \colorbox{c59}{the} \colorbox{c32}{spinal} \colorbox{c53}{column} \colorbox{c71}{.} \colorbox{c86}{)} \colorbox{c100}{<eos>} \\
------------------------K=10------------------------ \\
\small
use 0.844 can 0.816 used 0.801  \\
bottom 0.757 front 0.703 sides 0.691  \\
spinal 0.914 nerve 0.739 Spinal 0.700  \\
increases 0.766 decreasing 0.756 increasing 0.749  \\
devices 0.836 device 0.787 wireless 0.703  \\
symptoms 0.726 chronic 0.715 disease 0.692  \\
polymeric 0.674 hydrophilic 0.644 hydrophobic 0.636  \\
backboard 0.899 hoop 0.555 dunks 0.547  \\
column 0.898 columns 0.771 Column 0.584  \\
Kendrick 0.927 Lamar 0.620 Meek 0.611  \\
\normalsize
------------------------K=3------------------------ \\
\small
necessary 0.750 use 0.736 can 0.732  \\
spinal 0.801 thoracic 0.713 nerve 0.702  \\
backboard 0.771 ball 0.629 hoop 0.593  \\
\normalsize
------------------------K=1------------------------ \\
\small
tissue 0.667 prevent 0.659 pressure 0.642  \\
\normalsize

\colorbox{c58}{When} \colorbox{c21}{she} \colorbox{c44}{came} \colorbox{c74}{in} \colorbox{c72}{,} \colorbox{c21}{she} \colorbox{c49}{was} \colorbox{c46}{always} \colorbox{c77}{bound} \colorbox{c71}{to} \colorbox{c65}{be} \colorbox{c51}{loud} \colorbox{c72}{,} \colorbox{c59}{and} \colorbox{c55}{boisterous} \colorbox{c74}{.} \colorbox{c10}{Carrie} \colorbox{c47}{got} \colorbox{c61}{along} \colorbox{c60}{well} \colorbox{c63}{with} \colorbox{c66}{most} \colorbox{c76}{of} \colorbox{c71}{the} \colorbox{c58}{waitresses} \colorbox{c72}{,} \colorbox{c66}{most} \colorbox{c56}{especially} \colorbox{c41}{Vera} \colorbox{c30}{Louise} \colorbox{c60}{Gorman} \colorbox{c85}{-} \colorbox{c60}{Novak} \colorbox{c72}{,} \colorbox{c59}{and} \colorbox{c31}{Alice} \colorbox{c79}{Hyatt} \colorbox{c74}{.} \colorbox{c100}{<eos>} \\
------------------------K=10------------------------ \\
\small
really 0.893 know 0.877 think 0.869  \\
Carrie 0.901 Christina 0.727 Amanda 0.723  \\
daughter 0.816 mother 0.815 wife 0.781  \\
Carrie 0.908 Christina 0.748 Amanda 0.739  \\
came 0.730 went 0.722 had 0.711  \\
Maureen 0.750 Carolyn 0.749 Joanne 0.740  \\
endearing 0.670 downright 0.643 demeanor 0.632  \\
Vera 0.953 Aloe 0.639 vera 0.585  \\
actor 0.672 starring 0.650 comedy 0.639  \\
dancing 0.647 singing 0.598 raucous 0.593  \\
\normalsize
------------------------K=3------------------------ \\
\small
really 0.857 thought 0.853 never 0.846  \\
Carrie 0.881 Amanda 0.801 Rebecca 0.792  \\
waitress 0.596 hostess 0.595 maid 0.591  \\
\normalsize
------------------------K=1------------------------ \\
\small
knew 0.806 she 0.793 thought 0.788  \\
\normalsize

\colorbox{c76}{The} \colorbox{c34}{station} \colorbox{c47}{building} \colorbox{c66}{is} \colorbox{c40}{located} \colorbox{c67}{in} \colorbox{c63}{the} \colorbox{c57}{district} \colorbox{c71}{of} \colorbox{c100}{<unk>} \colorbox{c75}{.} \colorbox{c81}{These} \colorbox{c48}{services} \colorbox{c48}{operate} \colorbox{c70}{on} \colorbox{c63}{the} \colorbox{c58}{Eifel} \colorbox{c35}{Railway} \colorbox{c86}{(} \colorbox{c100}{<unk>} \colorbox{c82}{)} \colorbox{c75}{.} \colorbox{c100}{<eos>} \\
------------------------K=10------------------------ \\
\small
station 0.989 stations 0.847 Station 0.756  \\
Eifel 0.855 Harz 0.673 Cochem 0.642  \\
railway 0.820 railways 0.794 trains 0.782  \\
Germany 0.813 Berlin 0.766 Munich 0.751  \\
north 0.885 south 0.877 east 0.869  \\
building 0.867 buildings 0.794 construction 0.706  \\
located 0.696 operated 0.669 operates 0.668  \\
line 0.877 lines 0.739 Line 0.712  \\
Railway 0.751 Rail 0.622 Railways 0.591  \\
services 0.909 service 0.879 provider 0.708  \\
\normalsize
------------------------K=3------------------------ \\
\small
station 0.918 stations 0.807 railway 0.779  \\
located 0.802 area 0.770 situated 0.734  \\
Aachen 0.706 Eifel 0.701 Freiburg 0.661  \\
\normalsize
------------------------K=1------------------------ \\
\small
station 0.853 railway 0.834 stations 0.748  \\
\normalsize


\colorbox{c76}{Alfred} \colorbox{c100}{<unk>} \colorbox{c100}{<unk>} \colorbox{c77}{(} \colorbox{c68}{born} \colorbox{c53}{January} \colorbox{c71}{22} \colorbox{c79}{,} \colorbox{c61}{1965} \colorbox{c77}{)} \colorbox{c88}{is} \colorbox{c88}{a} \colorbox{c63}{Ghanaian} \colorbox{c66}{businessman} \colorbox{c82}{and} \colorbox{c88}{a} \colorbox{c51}{former} \colorbox{c41}{Honorary} \colorbox{c39}{Vice} \colorbox{c45}{Consul} \colorbox{c79}{of} \colorbox{c51}{Austria} \colorbox{c90}{to} \colorbox{c50}{Ghana} \colorbox{c82}{and} \colorbox{c88}{a} \colorbox{c76}{leading} \colorbox{c59}{member} \colorbox{c79}{of} \colorbox{c79}{the} \colorbox{c49}{National} \colorbox{c45}{Democratic} \colorbox{c49}{Congress} \colorbox{c88}{.} \colorbox{c100}{<eos>} \\
------------------------K=10------------------------ \\
\small
Ghana 0.928 Zambia 0.807 Cameroon 0.796  \\
Committee 0.824 Council 0.740 Commission 0.733  \\
election 0.810 elections 0.788 elected 0.774  \\
Austria 0.923 Germany 0.793 Austrian 0.739  \\
February 0.868 2011 0.865 2012 0.858  \\
Consul 0.898 consul 0.761 consular 0.596  \\
1995 0.970 1994 0.970 1993 0.969  \\
Party 0.886 party 0.707 Parties 0.649  \\
University 0.858 College 0.728 Graduate 0.727  \\
retired 0.575 born 0.572 emeritus 0.543  \\
\normalsize
------------------------K=3------------------------ \\
\small
President 0.778 Chairman 0.765 Committee 0.760  \\
Ghana 0.924 Zambia 0.808 Cameroon 0.806  \\
1999 0.956 1998 0.953 1997 0.951  \\
\normalsize
------------------------K=1------------------------ \\
\small
President 0.723 Affairs 0.664 Minister 0.658  \\
\normalsize


\colorbox{c35}{ISBN} \colorbox{c58}{0} \colorbox{c71}{-} \colorbox{c81}{8063} \colorbox{c71}{-} \colorbox{c66}{1367} \colorbox{c71}{-} \colorbox{c66}{6} \colorbox{c43}{Winthrop} \colorbox{c75}{,} \colorbox{c45}{John} \colorbox{c80}{.} \colorbox{c43}{Winthrop} \colorbox{c74}{'s} \colorbox{c47}{Journal} \colorbox{c75}{,} \colorbox{c30}{History} \colorbox{c79}{of} \colorbox{c44}{New} \colorbox{c47}{England} \colorbox{c58}{1630} \colorbox{c71}{-} \colorbox{c57}{1649} \colorbox{c80}{.} \colorbox{c44}{New} \colorbox{c41}{York} \colorbox{c75}{,} \colorbox{c50}{NY} \colorbox{c66}{:} \colorbox{c44}{Charles} \colorbox{c50}{Scribner} \colorbox{c74}{'s} \colorbox{c57}{Sons} \colorbox{c75}{,} \colorbox{c45}{1908} \colorbox{c80}{.} \colorbox{c100}{<eos>} \\
------------------------K=10------------------------ \\
\small
New 0.936 York 0.915 NY 0.807  \\
J. 0.847 R. 0.810 D. 0.807  \\
ISBN 0.934 Paperback 0.821 Hardcover 0.803  \\
History 0.830 Historical 0.694 War 0.681  \\
0 0.933 1 0.739 3 0.663  \\
Winthrop 0.926 Endicott 0.696 Amherst 0.672  \\
1985 0.840 1981 0.836 1982 0.834  \\
University 0.901 College 0.714 Northwestern 0.692  \\
England 0.875 London 0.718 Britain 0.680  \\
842 0.838 794 0.835 782 0.831  \\
\normalsize
------------------------K=3------------------------ \\
\small
William 0.841 J. 0.789 Robert 0.779  \\
New 0.887 York 0.860 NY 0.727  \\
1626 0.685 1684 0.676 1628 0.675  \\
\normalsize
------------------------K=1------------------------ \\
\small
William 0.686 York 0.676 Charles 0.643  \\
\normalsize

\colorbox{c74}{The} \colorbox{c63}{commune} \colorbox{c81}{is} \colorbox{c79}{represented} \colorbox{c83}{in} \colorbox{c79}{the} \colorbox{c76}{Senate} \colorbox{c74}{by} \colorbox{c62}{Soledad} \colorbox{c64}{Alvear} \colorbox{c76}{(} \colorbox{c82}{PDC} \colorbox{c77}{)} \colorbox{c85}{and} \colorbox{c51}{Pablo} \colorbox{c100}{<unk>} \colorbox{c76}{(} \colorbox{c83}{UDI} \colorbox{c77}{)} \colorbox{c84}{as} \colorbox{c76}{part} \colorbox{c82}{of} \colorbox{c79}{the} \colorbox{c69}{8th} \colorbox{c71}{senatorial} \colorbox{c70}{constituency} \colorbox{c76}{(} \colorbox{c47}{Santiago} \colorbox{c74}{-} \colorbox{c81}{East} \colorbox{c77}{)} \colorbox{c82}{.} \colorbox{c74}{Haha} \colorbox{c60}{Sound} \colorbox{c81}{is} \colorbox{c79}{the} \colorbox{c75}{second} \colorbox{c49}{album} \colorbox{c74}{by} \colorbox{c79}{the} \colorbox{c86}{British} \colorbox{c70}{indie} \colorbox{c82}{electronic} \colorbox{c67}{band} \colorbox{c77}{Broadcast} \colorbox{c82}{.} \colorbox{c100}{<eos>} \\
------------------------K=10------------------------ \\
\small
album 0.919 albums 0.844 songs 0.830  \\
constituency 0.810 election 0.773 elections 0.757  \\
released 0.931 release 0.847 releases 0.783  \\
Santiago 0.859 Juan 0.753 Luis 0.738  \\
Sound 0.890 Audio 0.739 Sounds 0.671  \\
February 0.881 2011 0.878 2010 0.877  \\
Jorge 0.687 Miguel 0.684 Pablo 0.683  \\
Alvear 0.738 Altamirano 0.563 Ruperto 0.552  \\
commune 0.939 communes 0.800 Commune 0.660  \\
\# 0.986 Item 0.523 1 0.507  \\
\normalsize
------------------------K=3------------------------ \\
\small
commune 0.718 communes 0.638 La 0.596  \\
album 0.948 albums 0.865 songs 0.796  \\
election 0.814 elections 0.791 electoral 0.745  \\
\normalsize
------------------------K=1------------------------ \\
\small
album 0.925 albums 0.818 Album 0.745  \\
\normalsize


\colorbox{c70}{As} \colorbox{c72}{a} \colorbox{c71}{result} \colorbox{c78}{,} \colorbox{c64}{the} \colorbox{c51}{Hellfire} \colorbox{c59}{Club} \colorbox{c55}{believed} \colorbox{c61}{that} \colorbox{c65}{it} \colorbox{c63}{would} \colorbox{c67}{be} \colorbox{c75}{in} \colorbox{c61}{their} \colorbox{c74}{best} \colorbox{c72}{interests} \colorbox{c71}{to} \colorbox{c54}{summon} \colorbox{c64}{the} \colorbox{c54}{Phoenix} \colorbox{c71}{and} \colorbox{c84}{merge} \colorbox{c65}{it} \colorbox{c71}{with} \colorbox{c59}{Jean} \colorbox{c53}{Grey} \colorbox{c87}{via} \colorbox{c72}{a} \colorbox{c70}{ritual} \colorbox{c80}{.} \colorbox{c100}{<eos>} \\
------------------------K=10------------------------ \\
\small
want 0.886 way 0.875 sure 0.871  \\
attack 0.722 kill 0.708 enemy 0.708  \\
beings 0.703 manifestation 0.690 spiritual 0.685  \\
disappeared 0.710 apparently 0.681 initially 0.678  \\
Evil 0.719 Darkness 0.694 Demon 0.693  \\
Phoenix 0.950 Tucson 0.688 Tempe 0.658  \\
Hellfire 0.932 hellfire 0.623 Brimstone 0.530  \\
Grey 0.956 Gray 0.788 Blue 0.771  \\
Jean 0.912 Pierre 0.767 Jacques 0.736  \\
Club 0.903 club 0.804 clubs 0.680  \\
\normalsize
------------------------K=3------------------------ \\
\small
even 0.836 somehow 0.823 because 0.816  \\
Hellfire 0.814 Scourge 0.606 Goblin 0.588  \\
Blue 0.738 Grey 0.730 Red 0.693  \\
\normalsize
------------------------K=1------------------------ \\
\small
somehow 0.780 even 0.769 nothing 0.747  \\
\normalsize

\colorbox{c70}{Skeletal} \colorbox{c46}{problems} \colorbox{c78}{,} \colorbox{c22}{infection} \colorbox{c78}{,} \colorbox{c58}{and} \colorbox{c21}{tumors} \colorbox{c51}{can} \colorbox{c63}{also} \colorbox{c42}{affect} \colorbox{c59}{the} \colorbox{c43}{growth} \colorbox{c62}{of} \colorbox{c59}{the} \colorbox{c32}{leg} \colorbox{c78}{,} \colorbox{c51}{sometimes} \colorbox{c59}{giving} \colorbox{c55}{rise} \colorbox{c59}{to} \colorbox{c62}{a} \colorbox{c57}{one} \colorbox{c94}{-} \colorbox{c73}{sided} \colorbox{c51}{bow} \colorbox{c94}{-} \colorbox{c100}{<unk>} \colorbox{c67}{.} \colorbox{c100}{<eos>} \\
------------------------K=10------------------------ \\
\small
symptoms 0.851 disease 0.826 chronic 0.818  \\
often 0.857 usually 0.854 may 0.851  \\
infection 0.849 infections 0.807 infected 0.772  \\
tumors 0.867 tumours 0.834 tumor 0.791  \\
epithelial 0.676 epithelium 0.672 upregulation 0.667  \\
increasing 0.805 increased 0.799 increases 0.798  \\
legs 0.737 shoulders 0.716 fingers 0.715  \\
leg 0.909 legs 0.785 thigh 0.750  \\
mammalian 0.666 gene 0.664 genes 0.654  \\
bow 0.899 bows 0.775 sash 0.574  \\
\normalsize
------------------------K=3------------------------ \\
\small
affect 0.769 significant 0.755 decrease 0.741  \\
disease 0.795 infection 0.782 infections 0.757  \\
epithelial 0.691 extracellular 0.686 epithelium 0.685  \\
\normalsize
------------------------K=1------------------------ \\
\small
disease 0.764 abnormal 0.751 tissue 0.743  \\
\normalsize

\colorbox{c100}{<unk>} \colorbox{c83}{is} \colorbox{c81}{composed} \colorbox{c82}{of} \colorbox{c82}{the} \colorbox{c81}{:} \colorbox{c51}{Jack} \colorbox{c54}{Carty} \colorbox{c94}{may} \colorbox{c89}{refer} \colorbox{c89}{to} \colorbox{c81}{:} \colorbox{c51}{Jack} \colorbox{c54}{Carty} \colorbox{c74}{(} \colorbox{c46}{musician} \colorbox{c75}{)} \colorbox{c74}{(} \colorbox{c46}{born} \colorbox{c50}{1987} \colorbox{c75}{)} \colorbox{c78}{,} \colorbox{c48}{Australian} \colorbox{c46}{musician} \colorbox{c51}{Jack} \colorbox{c54}{Carty} \colorbox{c74}{(} \colorbox{c45}{rugby} \colorbox{c63}{union} \colorbox{c75}{)} \colorbox{c74}{(} \colorbox{c46}{born} \colorbox{c52}{1992} \colorbox{c75}{)} \colorbox{c78}{,} \colorbox{c45}{rugby} \colorbox{c63}{union} \colorbox{c60}{player} \colorbox{c79}{from} \colorbox{c42}{Ireland} \colorbox{c42}{John} \colorbox{c54}{Carty} \colorbox{c74}{(} \colorbox{c73}{disambiguation} \colorbox{c75}{)} \colorbox{c100}{<eos>} \\
------------------------K=10------------------------ \\
\small
February 0.910 April 0.906 June 0.904  \\
States 0.746 American 0.745 United 0.735  \\
Australian 0.848 Zealand 0.749 Australia 0.729  \\
born 0.880 Born 0.686 married 0.596  \\
band 0.598 album 0.596 music 0.583  \\
Carty 0.914 Kelleher 0.621 O'Mahony 0.619  \\
1977 0.967 1978 0.964 1974 0.963  \\
football 0.786 player 0.740 soccer 0.740  \\
union 0.841 unions 0.698 Unions 0.631  \\
Jack 0.800 Jim 0.727 Tom 0.715  \\
\normalsize
------------------------K=3------------------------ \\
\small
1975 0.740 1981 0.738 1978 0.736  \\
Ireland 0.910 Irish 0.782 Dublin 0.747  \\
rugby 0.766 football 0.759 soccer 0.718  \\
\normalsize
------------------------K=1------------------------ \\
\small
England 0.609 Rugby 0.600 Wales 0.596  \\
\normalsize

\colorbox{c73}{He} \colorbox{c54}{designed} \colorbox{c68}{a} \colorbox{c58}{system} \colorbox{c57}{of} \colorbox{c35}{streets} \colorbox{c54}{which} \colorbox{c57}{generally} \colorbox{c69}{followed} \colorbox{c54}{the} \colorbox{c66}{contours} \colorbox{c57}{of} \colorbox{c54}{the} \colorbox{c28}{area} \colorbox{c68}{'s} \colorbox{c53}{topography} \colorbox{c70}{.} \colorbox{c48}{Residential} \colorbox{c27}{neighborhoods} \colorbox{c70}{stretched} \colorbox{c61}{out} \colorbox{c64}{from} \colorbox{c68}{a} \colorbox{c40}{commercial} \colorbox{c56}{and} \colorbox{c46}{service} \colorbox{c84}{-} \colorbox{c49}{sector} \colorbox{c65}{core} \colorbox{c70}{.} \colorbox{c100}{<eos>} \\
------------------------K=10------------------------ \\
\small
creating 0.737 incorporate 0.726 developing 0.720  \\
north 0.861 south 0.859 east 0.855  \\
sector 0.874 sectors 0.790 economic 0.746  \\
neighborhoods 0.840 streets 0.775 neighbourhoods 0.749  \\
City 0.745 Riverside 0.726 Heights 0.709  \\
buildings 0.691 brick 0.672 building 0.658  \\
topography 0.817 vegetation 0.708 forested 0.702  \\
service 0.889 services 0.809 Service 0.663  \\
Building 0.742 Construction 0.613 Project 0.581  \\
1930 0.856 1920s 0.826 1929 0.815  \\
\normalsize
------------------------K=3------------------------ \\
\small
development 0.739 significant 0.720 providing 0.719  \\
streets 0.831 city 0.793 neighborhoods 0.786  \\
County 0.669 Riverside 0.662 City 0.649  \\
\normalsize
------------------------K=1------------------------ \\
\small
buildings 0.765 area 0.761 areas 0.753  \\
\normalsize

==> AAAI 2021 NSD/more_exp.tex <==
In the main paper, we show that multi-facet embeddings can improve the estimation of symmetric relations like similarity. To know whether they are also useful in asymmetric relations like entailment, we test our method on a hypernym detection dataset in Section~\ref{sec:hyper}.

Due to the page limits, we cannot present all of our results in the main paper, so we put more comprehensive analyses for sentence similarity tasks in Section~\ref{sec:sent_sim_more}, for extractive summarization in Section~\ref{sec:sum_more}, and for phrase similarity tasks in Section~\ref{sec:phrase_sim_more}. We also present the results of BERT Large model in Section~\ref{sec:bert_large} as a reference. Section~\ref{sec:good_example_STS} and~\ref{sec:good_example_sum} provide some motivating examples for a sentence similarity task and for the extractive summarization, respectively. 





% and sentence entailment task in Section~\ref{sec:sent_entail}
%/.. our methods
%explore the 
%In addition to symmetric scoring functions like similarity, we test our method



\subsection{Unsupervised Hypernymy Detection}
\label{sec:hyper}
We apply our model to HypeNet~\citep{hypenet}, an unsupervised hypernymy detection dataset, based on the assumption that the co-occurring words of a phrase are often less related to some of its hyponyms. For instance, \emph{animal} is a hypernym of \emph{brown dog}. \emph{flies} is a co-occurring word of \emph{animal} which is less related to \emph{brown dog}. 

%the co-occurring words of \emph{brown dog} are often related to \emph{animal}. On the other hand,

%a more specific phrase usually indicates that its

Accordingly, the predicted codebook embeddings of a hyponym $S^{hypo}_q$ (e.g., \emph{brown dog}), which cluster the embeddings of co-occurring words (e.g., \emph{eats}), often reconstruct the embeddings of its hypernym $S^{hyper}_q$ (e.g., \emph{animal}) better than the other way around (e.g., the embedding of \emph{flies} cannot reconstruct the embeddings of \emph{brown dog} well).  That is, $Er(\bm{\widehat{F}_u(S^{hypo}_q)}, \bm{W(S^{hyper}_q)})$ is smaller than $Er(\bm{\widehat{F}_u(S^{hyper}_q)}, \bm{W(S^{hypo}_q)})$).

Based on the assumption, our asymmetric scoring function is defined as

\vspace{-4mm}
\footnotesize
\begin{align}
 & \text{Diff}(S^{hyper}_q, S^{hypo}_q)  = Er(\bm{\widehat{F}_u(S^{hyper}_q)}, \bm{W(S^{hypo}_q)}) \nonumber \\
 & - Er(\bm{\widehat{F}_u(S^{hypo}_q)}, \bm{W(S^{hyper}_q)}).
 \end{align}
\normalsize
where Er function is defined in~\refeqerdot
%where $S^{hyper}_q$ and $S^{hypo}_q$ are the query sequences of hypernym and hyponym respectively, and $\bm{W(S_q)} = [\underline{\vw}_{i}]_{i=1...|S_q|}$. 
%$Asym(S^{hyper}_q, S^{hypo}_q)$ is more likely to be positive because the co-occurring distribution of hyponym $S^{hypo}_q$ should reconstruct the word embeddings of hypernym $W(S^{hyper}_q)$ better than the other way around.
%(i.e., $ Er(\widehat{F}_u(S^{hypo}_q), W(S^{hyper}_q))<Er(\widehat{F}_u(S^{hyper}_q), W(S^{hypo}_q))$ ).

%using the codebook vectors 

%assuming that possible co-occurring words of hyponym is more likely to be close to its hypernym.

The AUC of detecting hypernym among other relations and accuracy of detecting the hypernym direction are compared in Table~\ref{tb:phrase_hyper}. Our methods outperform baselines, which only provide symmetric similarity measurement, and \textbf{Ours (K=1)} performs similarly compared with \textbf{Ours (K=10)}.



%to show that it can also be used to measure asymmetric relation.

%The possible co-occurring words of hypernym have more possibility, so their distribution is less likely to cover each of its hyponyms. On the contrary. the 


%AUC means area under the precision and recall curve of detecting hypernym phrases


%\begin{table}[t!]
%\scalebox{0.95}{
%\begin{tabular}{|cc|c|c|}
%\hline
%\multicolumn{2}{|c|}{Method} & Dev & Test \\ \hline
%Avg & \multicolumn{1}{|c|}{ELMo} & 50.5 & 50.6  \\ \hline
%Avg & \multicolumn{1}{|c|}{BERT} & 42.9 & 44.0  \\ \hline
%\multirow{3}{*}{Avg} & \multicolumn{1}{|c|}{GloVe} & 48.0 &	49.5   \\ 
% & \multicolumn{1}{|c|}{Our a K1} & 49.2 &	49.3  \\ 
% & \multicolumn{1}{|c|}{Our a K10} & 50.4 &	50.1 \\ \hline
% \multirow{3}{*}{Asym} & \multicolumn{1}{|c|}{GloVe} &  68.9 &	68.0   \\ 
% & \multicolumn{1}{|c|}{Our a K1} & 68.9 & 68.5  \\ 
% & \multicolumn{1}{|c|}{Our a K10} & \textbf{69.8} & \textbf{69.4} \\ \hline
%\end{tabular}
%}
%\centering
%\caption{Comparison of F1 (\%) in our sentence entailment task in SNLI.}
%\label{tb:sent_entail}
%\end{table}

%\subsection{Unsupervised Sentence Entailment}
%\label{sec:sent_entail}
%We merge the contradiction and neutral labels in Stanford natural language inference (SNLI) dataset~\citep{bowman2015large}, and convert the problem into a binary classification task (i.e., determine whether premise entails hypothesis). Furthermore, we assume that each premise only entails one hypothesis among the hypothesis candidates, then the problem is simplified as identifying the entailment hypothesis of each premise.

%to simplify the problem.
%, there is only one hypothesis 

%We hypothesize that the sentence pairs with entailment relations will be more similar to each other, so the first scoring function we try, \textbf{Avg}, computes the cosine similarity between average (contextualized) word embeddings and label the hypothesis which is most similar to the premise as entailment. 

%We observe that lots of entailed hypotheses are a more abstract and shorter version of its premises (e.g., \emph{I see a brown dog in the yard} implies \emph{I see an animal}), so we also try an asymmetric similarity function, \textbf{Asym}, that finds the most similar word in premise for each word in the hypothesis (e.g., find the word \emph{dog} for the word \emph{animal}) and averages their cosine similarity across all the words in the hypothesis. 
%However, we discover that the similarity between sentence pairs with different premises are not well aligned.

%We apply our word importance estimation in~\refeqatt~to above two scoring functions and we can see in Table~\ref{tb:sent_entail} that the important weighting derived from multi-facet embeddings improves the F1 score of detecting entailed hypothesis for each premise in both \textbf{Avg} and \textbf{Asym} scoring functions.
%compare its performance with 
\begin{table}[t!]
\scalebox{1}{
\begin{tabular}{|c|c|cc|cc|}
\hline
\multicolumn{2}{|c|}{Method} & \multicolumn{2}{|c|}{Dev} & \multicolumn{2}{|c|}{Test}  \\ \hline
Model & Score& AUC & Acc  & AUC & Acc \\ \hline
\multirow{2}{*}{BERT} & CLS & 20.6 & 50 & 21.3 & 50 \\ 
& Avg & 25.6 & 50 & 25.6 & 50 \\ \hline
GloVe & Avg & 17.4 & 50 & 17.7 & 50 \\ 
%SBOW (AL1) & & &  & \\ \hline
%DIVE (AL1) & & &  & \\ \hline
Our c K10 & Diff & \textbf{29.4} & 78.9  & \textbf{29.6} & 79.1 \\ 
Our c K1 & Diff & 29.3 & \textbf{82.7} & \textbf{29.6}  & \textbf{81.0} \\ \hline
\end{tabular}
}
\centering
\caption{Hypernym detection performances in the development and test set of HypeNet. AUC (\%) refers to the area under precision and recall curve, which measures the quality of retrieving hypernym phrases. Acc (\%) means the accuracy of predicting specificity given a pair of hypernym phrases.}
\label{tb:phrase_hyper}
\end{table}

\begin{table}[t!]
\scalebox{0.8}{
\begin{tabular}{|cc|cc|cc|}
\hline
\multicolumn{2}{|c|}{Method} & \multicolumn{2}{|c|}{Dev} & \multicolumn{2}{|c|}{Test} \\ \hline
\multicolumn{1}{|c|}{Score} & Model & All & Low & All & Low   \\ \hline
\multicolumn{1}{|c|}{Cosine} & Skip-thought & 43.2 & 28.1 & 30.4 & 21.2 \\ \hline
\multicolumn{1}{|c|}{Avg} & ELMo & 65.6 &	47.4 &	54.2&	44.1 \\ \hline
\multirow{3}{*}{Prob\_avg} & \multicolumn{1}{|c|}{ELMo} & 70.3 &	54.6 &	60.4 & 54.2 \\ 
 & \multicolumn{1}{|c|}{Our a (GloVe) K1} & 69.3 &	54.1 & 60.8 & 55.8 \\
 & \multicolumn{1}{|c|}{Our a (GloVe) K10} & 70.5 &	55.9 &	61.1 & 56.6 \\ \hline
\multicolumn{1}{|c|}{Avg} & \multirow{2}{*}{BERT} & 62.3 & 42.1 & 51.2 & 39.1 \\ 
\multicolumn{1}{|c|}{Prob\_avg} &  & 72.1 & 57.0 & 57.8 & 55.1 \\ \hline
\multirow{3}{*}{Avg} & \multicolumn{1}{|c|}{Sent2Vec} & 71.9 & 51.2 & 63.6 & 46.0 \\
& \multicolumn{1}{|c|}{Our a (GloVe) K10} & 76.1 & 62.9 & \textbf{71.5} & \textbf{62.7} \\
& \multicolumn{1}{|c|}{Our a (GloVe) K1} & 72.0 & 56.1 & 66.8 & 55.7 \\ \hline
\multirow{5}{*}{SC} & \multicolumn{1}{|c|}{NNSC clustering K10} & 38.6&	37.8&	25.4&	38.9 \\
 & \multicolumn{1}{|c|}{Our c (w2v) K10} & 54.7&	38.8&	43.9&	36.0 \\ 
  & \multicolumn{1}{|c|}{Our c (k-means) K10} & 37.8&	25.9&	29.5&	19.7 \\ 
  & \multicolumn{1}{|c|}{Our c (LSTM) K10} & 58.9 & 49.2 & 49.8 & 46.4 \\ 
  & \multicolumn{1}{|c|}{Our c (GloVe) K10} & 63.0 & 51.8 & 52.6 & 47.8 \\ \hline
\multirow{2}{*}{Prob\_WMD} & \multicolumn{1}{|c|}{w2v} & 72.9&	56.6&	62.1&	54.0 \\
 & \multicolumn{1}{|c|}{Our a (w2v) K10} & 73.6&	60.1&	63.5&	57.8 \\ \hline
 \multirow{2}{*}{Prob\_avg} & \multicolumn{1}{|c|}{w2v} & 68.3&	53.7&	54.3&	50.9 \\
 & \multicolumn{1}{|c|}{Our a (w2v) K10} & 68.3&	56.8&	55.1&	53.1 \\ \hline
 \multirow{2}{*}{SIF$\dagger$} & \multicolumn{1}{|c|}{w2v} & 70.5&	56.9&	59.4&	54.7 \\
 & \multicolumn{1}{|c|}{Our a (w2v) K10} & 71.6&	60.9&	61.3&	57.6 \\ \hline
\multirow{4}{*}{Prob\_WMD} & \multicolumn{1}{|c|}{GloVe} & 75.1 & 59.6 &	63.1 &	52.5 \\
  & \multicolumn{1}{|c|}{Our a (k-means) K10} & 72.5&	57.9&	60.3&	49.9 \\ 
 & \multicolumn{1}{|c|}{Our a (LSTM) K10} & \textbf{76.3}&	\textbf{63.2}&	65.8&	57.4 \\ 
 & \multicolumn{1}{|c|}{Our a (GloVe) K10} & 76.2 & 62.6 & 66.1 & 58.1 \\ \hline
\multirow{4}{*}{Prob\_avg} & \multicolumn{1}{|c|}{GloVe} & 70.7 & 56.6 & 59.2	& 54.8 \\
  & \multicolumn{1}{|c|}{Our a (k-means) K10} & 66.6&	53.4&	55.8&	51.8 \\ 
 & \multicolumn{1}{|c|}{Our a (LSTM) K10} & 71.7 & 60.1 & 61.3 & 58.3 \\ 
 & \multicolumn{1}{|c|}{Our a (GloVe) K10} & 72.0 & 60.5 & 61.4 & 59.3 \\ \hline
 \multirow{4}{*}{SIF$\dagger$} & \multicolumn{1}{|c|}{GloVe} & 75.1 & 65.7 & 63.2 & 58.1 \\
  & \multicolumn{1}{|c|}{Our a (k-means) K10} & 71.5&	62.3&	61.5&	57.2 \\ 
 & \multicolumn{1}{|c|}{Our a (LSTM) K10} & 74.6 & 66.9 & 64.3 & 60.9 \\ 
 & \multicolumn{1}{|c|}{Our a (GloVe) K10} &\textbf{75.2} & \textbf{67.6} & \textbf{64.6} & \textbf{62.2} \\ \hline
\end{tabular}
}
\centering
\caption{The Pearson correlation (\%) in STS benchmarks. w2v means Word2Vec. Our * (k-means) means using the k-means loss rather than the NNSC loss. Our * (LSTM) means replacing the transformers in our encoder with bi-LSTM and replacing our transformer decoder with LSTM. Other abbreviations and symbols share the same meaning in Table~\reftbsts.}
\label{tb:STS_more}
\end{table}

\begin{table*}[t!]
\scalebox{0.8}{
\begin{tabular}{|ccc|ccc||ccc||cccc|}
\hline
\multicolumn{3}{|c|}{Dataset} & \multicolumn{3}{c||}{Prob\_avg} & \multicolumn{2}{|c|}{Prob\_WMD} & WMD & \multicolumn{4}{|c|}{Avg} \\ \hline
Category & Data & Year & Our a K10 & GloVe & Our a K1 & Our a K10 & GloVe & GloVe & w2v & BERT & ELMo & ST \\ \hline
\multirow{5}{*}{forum} &	deft-forum & 2014 & \textbf{40.3}&	33.2&	35.6&	\textbf{41.4}&	33.3&	28.5&	33.9&	25.6&	\textbf{35.9}&	22.5 \\
 & answers-forums&2015&\textbf{53.9}&49.6&43.4&\textbf{63.7}&61.4&48.7&51.2&55.1&\textbf{56.0}&36.8\\
& answer-answer&2016&\textbf{39.5}&34.1&33.1&\textbf{48.9}&45.0&46.4&31.0&50.4&\textbf{58.2}&32.3\\
& question-question&2016&\textbf{63.5}&61.4&60.1&\textbf{66.9}&62.6&28.7&\textbf{53.7}&44.9&38.4&42.3\\
& belief&2015&\textbf{58.6}&57.2&53.5&\textbf{67.8}&66.9&62.6&63.8&62.8&\textbf{71.1}&38.5\\ \hline
\multirow{5}{*}{news} & surprise.SMTnews&2012&\textbf{56.7}&50.9&54.4&\textbf{55.9}&49.0&48.4&48.7&\textbf{56.8}&55.1&44.2\\
& headlines&2013&\textbf{57.9}&55.9&53.3&\textbf{67.5}&66.2&59.6&54.8&55.1&\textbf{59.7}&44.6\\
& headlines&2014&\textbf{53.0}&51.2&49.1&\textbf{61.8}&59.9&53.3&50.4&53.2&\textbf{54.2}&41.6\\
& headlines&2015&\textbf{54.7}&51.8&49.8&\textbf{65.4}&63.6&59.1&51.8&53.3&\textbf{59.2}&47.6\\
& headlines&2016&\textbf{53.9}&52.0&49.8&\textbf{65.6}&64.6&62.6&50.3&\textbf{58.0}&57.3&46.6\\ \hline
\multirow{4}{*}{definition} & surprise.OnWN&2012&\textbf{66.6}&64.0&63.6&\textbf{69.8}&68.2&65.3&63.3&60.3&\textbf{68.8}&33.5 \\
& OnWN&2013&\textbf{69.8}&68.6&63.6&\textbf{65.0}&61.8&35.6&\textbf{63.8}&59.7&44.8&21.1 \\
& OnWN&2014&\textbf{75.9}&74.8&72.7&\textbf{73.8}&71.9&52.5&\textbf{74.5}&71.0&61.1&31.1 \\
& FNWN&2013&\textbf{39.4}&38.6&38.9&45.7&\textbf{46.0}&40.1&28.0&36.5&\textbf{38.1}&11.0 \\ \hline
\multirow{3}{*}{captions} & MSRvid&2012&\textbf{81.5}&81.2&80.5&\textbf{80.4}&78.3&46.3&\textbf{76.0}&52.3&63.0&54.3 \\
&images&2014&\textbf{76.9}&74.6&75.5&\textbf{78.1}&75.1&57.3&\textbf{72.1}&55.4&64.9&62.8 \\
&images&2015&76.1&\textbf{76.5}&74.5&\textbf{82.2}&81.8&67.3&72.8&66.3&\textbf{73.3}&29.5 \\ \hline
\multirow{2}{*}{education} & answers-students&2015&53.3&\textbf{54.7}&52.5&66.4&68.5&\textbf{70.4}&\textbf{64.0}&62.8&60.4&41.5 \\
 & plagiarism&2016&72.1&\textbf{74.4}&72.2&78.5&\textbf{79.1}&71.2&74.0&76.6&\textbf{78.4}&53.6 \\ \hline
\multirow{2}{*}{out of domain} & deft-news&2014&62.4&\textbf{65.6}&59.0&63.9&\textbf{65.2}&55.5&58.9&\textbf{73.3}&72.6&43.8 \\
& tweet-news&2014&64.0&\textbf{66.2}&60.1&71.1&\textbf{72.7}&70.5&69.7&66.5&\textbf{72.0}&53.1 \\ \hline
\multirow{3}{*}{similar} & MSRpar&2012&34.6&\textbf{43.4}&36.2&48.0&\textbf{53.2}&49.0&37.2&\textbf{40.5}&34.0&24.5 \\
 & SMTeuroparl&2012&52.3&\textbf{54.4}&42.8&\textbf{53.6}&53.3&51.3&\textbf{51.8}&46.0&46.8&28.4 \\
 & postediting&2016&65.4&\textbf{66.8}&63.5&78.9&\textbf{79.9}&78.0&74.3&79.1&\textbf{80.2}&57.4 \\ \hline
\multirow{12}{*}{STS} & All & 2012&68.4&\textbf{68.5}&68.0&\textbf{66.8}&64.9&40.0&\textbf{60.5}&32.5&44.1&6.6 \\
& All & 2013&\textbf{64.1}&62.0&58.9&\textbf{66.5}&64.2&47.3&\textbf{58.5}&57.4&54.1&36.3 \\
& All&2014&\textbf{58.6}&56.1&52.7&\textbf{61.4}&58.8&39.2&\textbf{56.1}&53.6&52.4&25.0 \\
& All&2015&\textbf{59.3}&56.8&54.2&\textbf{71.1}&70.1&58.1&\textbf{61.6}&58.1&57.4&25.8 \\
& All&2016&\textbf{56.9}&53.7&52.4&\textbf{66.7}&62.8&49.6&52.9&\textbf{60.4}&57.9&38.8 \\
& All&All&\textbf{61.4}&59.5&56.5&\textbf{66.8}&64.8&48.4&\textbf{59.1}&54.1&55.4&26.1 \\
& Low&2012&67.1&\textbf{67.9}&\textbf{67.9}&\textbf{60.8}&59.2&17.5&\textbf{57.5}&18.8&33.0&-2.0 \\
& Low&2013&\textbf{49.4}&45.1&44.3&\textbf{39.4}&32.7&10.5&\textbf{33.1}&31.5&27.4&22.9 \\
& Low&2014&\textbf{50.2}&45.1&43.5&\textbf{50.5}&45.5&22.3&43.5&\textbf{46.6}&40.4&29.4 \\ 
& Low&2015&\textbf{48.8}&45.3&43.8&\textbf{54.2}&50.9&33.4&\textbf{49.8}&38.2&41.3&18.7 \\ 
& Low&2016&\textbf{51.0}&45.1&44.5&\textbf{53.8}&46.3&21.7&\textbf{39.4}&36.4&32.4&21.6 \\
& Low&All&\textbf{51.2}&47.7&45.9&\textbf{52.3}&48.4&25.8&\textbf{45.9}&39.8&39.5&21.7 \\ \hline
\end{tabular}
}
\centering
\caption{Comparing Pearson correlation (\%) of different unsupervised methods from STS 2012 to STS 2016. We highlight the best performance in each of the three blocks.}
\label{tb:STS_all}
\end{table*}

\subsection{More Analysis on Sentence Similarity }
\label{sec:sent_sim_more}
We design more experiments and present the results in Table~\ref{tb:STS_more} and Table~\ref{tb:STS_all} in order to answer the following research questions.

\textbf{1. Is ignoring the order of co-occurring words effective in emphasizing the semantic side of the sentences?}

To answer this question, we replace our transformer encoder with bi-LSTM and our transformer decoder with LSTM. Then, this architecture becomes very similar to skip-thought~\citep{kiros2015skip} except that skip-thoughts decodes a sequence instead of a set, and we ignore the word order in the nearby sentences. As we can see in Table~\ref{tb:STS_more}, \textbf{Our c (LSTM) K10 SC} performs much better than \textbf{Skip-thought Cosine}, which compute the cosine similarity between their sentence embeddings. This result further justifies our approach of ignoring the order of co-occurring words in our NNSC loss.

%compare this variant of our method with skip-thought embeddings

%cosine similarity between skip-thought embeddings (\textbf{ST Cos})~\citep{kiros2015skip}

%We also test a variant of our method which uses a bi-LSTM as the encoder and a LSTM as the decoder.

%Its average validation loss (-0.1289) in~\refeqobj~ %~\eqref{eq:obj_func} 
%is significantly higher than that of the transformer alternative (-0.1439), and it performances on Table~\ref{tb:STS_more} are usually also worse. Notice the architecture of this variant is similar to skip-thoughts except that skip-thoughts decodes a sequence instead of a set. The variant significantly outperforms \textbf{ST Cos}, which further justifies our approach of ignoring the order of co-occurring words in our NNSC loss.

\textbf{2. Is our word importance estimation generally useful for composing (contextualized) word embedding models?}

We cannot apply our attention weights (i.e.,  \textbf{Our a}) to BERT because BERT uses word piece tokenization. Instead, we use the top layer of ELMo~\citep{ELMo} as the contextualized word embedding, apply $\frac{\alpha}{\alpha + p(w)}$ weighting multiplied with our attention weights in~\refeqatt. The results in Table~\ref{tb:STS_more} show that the performance of \textbf{ELMo Prob\_avg} could also be boosted by our attention weighting even though our model is trained on GloVe semantic space. The importance weights from multiple embeddings can also help boost the performance of a version of Sent2Vec~\citep{pgj2017unsup} that uses only unigram information.
%~derived from the multi-facet embeddings in the GloVe space

\textbf{3. Could our model be trained on word embedding space other than GloVe?}

First, we train Word2Vec~\citep{word2vec} (denoted as w2v) on the Wikipedia 2016 corpus. We then train our multi-facet embeddings to fit the Word2Vec embedding of co-occurring words in the Wikipedia 2016 corpus. The results in Table~\ref{tb:STS_more} show that \textbf{Our a (w2v) K10} improves the performance using different scoring functions as we did in GloVe space.
%, the same corpus we used to train our multi-facet embeddings
%repeat the experiments .
%w2v is trained in the same corpus (Wikipedia 2016).

\textbf{4. How well could clustering-based multi-facet embeddings perform on long text sequences such as sentences?}

Lots of the testing sentences in the STS benchmark are not observed in our training corpus. To test clustering-based multi-facet embeddings, we first average word embedding in every sentence into sentence embedding, and for each testing query sentence, we perform approximated nearest neighbor search using KDTree~\citep{bentley1975multidimensional} to retrieve 1000 most similar sentences. Then, we remove the stop words in the 1000 sentences and perform NNSC clustering on the rest of the words. Finally, we compute \textbf{SC} distance between two sets of cluster centers derived from testing sentence pairs and denote the baseline as \textbf{NNSC clustering K10 SC} in Table~\ref{tb:STS_more}. 

The testing time of this baseline is much slower than the proposed method due to the need for the nearest neighbor search, and its performance is also much worse. This result justifies our approach of predicting clustering centers directly to generate multi-facet embeddings.
%We can see that .

\textbf{5. How much better is NNSC loss compared with k-means loss?}

In the method section, we mention that we adopt NNSC rather than k-means in our loss because k-means loss cannot generate diverse cluster centers in all of the neural architectures (including transformers and bi-LSTMs) we tried. We hypothesize that the k-means loss does not stably encourage predicted clusters to play different roles for reconstructing the embeddings of observed co-occurring words. We present the much worse results of the model using k-means loss in Table~\ref{tb:STS_more} to justify our usage of NNSC in our loss.

%In this work, we adopt the relaxation because for all neural architectures (including transformers and LSTMs) we tried, the models using a NNSC loss learn to generate diverse $K$ cluster centers while the predicted cluster centers using the kmeans loss collapse to much fewer modes which cannot well capture the conditional co-occurrence distribution. We hypothesize that it is because a NNSC loss is smoother and easier to be optimized for a neural network, while finding the nearest cluster center in the kmeans loss does not stably encourage predicted clusters to play different roles for reconstructing the embeddings of observed co-occurring words.

\textbf{6. Could our method improve the similarity estimation of all kinds of datasets?}

In Table~\ref{tb:STS_all}, we compare the performance before and after applying our attention weights in the English part of STS 2012~\citep{agirre2012semeval}, 2013~\citep{agirre2013sem}, 2014~\citep{agirre2014semeval}, 2015~\citep{agirre2015semeval}, and 2016~\citep{agirre2016semeval}. We categorize each of the dataset in different years based on either its source (\emph{forum}, \emph{news}, \emph{definition}, \emph{caption}, and \emph{education}) or its characteristic (\emph{out of domain} or \emph{similar}). 

\emph{Out of domain} means the testing sentences are very different from our training corpus, Wikipedia 2016. \emph{deft-news} from STS 2014 is included in this category because all the sentences in the dataset are lowercased. \emph{Similar} means there are lots of pairs in the datasets whose two sentences have almost the identical meaning. 

From the Table~\ref{tb:STS_all}, we can see that \textbf{GloVe Prob\_avg} and \textbf{GloVe Prob\_WMD} perform well compare with other baselines, and the attention weights from our multi-facet embedding stably boost \textbf{GloVe Prob\_avg} and \textbf{GloVe Prob\_WMD} except in the categories \emph{education}, \emph{out of domain}, and \emph{similar}. Thus, we recommend adopting our method when the source of training and testing sentences are not too different from each other, and the task is not to identify duplicated sentences.

\textbf{7. Are supervised methods such as sentence-BERT sensitive to the training data?}

Table~\ref{tb:sentence_bert_details} compares the performance of sentence-BERT~\citep{reimers2019sentence} trained on different data sources. We observe that the performance of sentence-BERT could be degraded when the distribution of training data is very different from that of testing data. For example, Sentence-BERT also does not perform well when the training sentence pairs tend to be similar with each other (e.g., in \emph{postediting} and \emph{SMTeuroparl}) or come from a writing style that is different from the style of testing sentence pairs (e.g., \emph{tweet-news} and \emph{answers-students}). 

Furthermore, a supervised model trained by a limited amount of labels could perform worse than the unsupervised alternatives. For example, on STSB Dev, the weighted average of word embedding (Prob\_avg) outputted by the BERT base model outperforms the sentence-BERT trained by 100 labels on average. Sentence-BERT model trained by \emph{SMTeuroparl} is even worse than just averaging all the contextualized word embeddings in BERT on STSB Test.


\begin{table}[t!]
\scalebox{0.9}{
\begin{tabular}{|cc|cc|cc|}
\hline
\multicolumn{2}{|c|}{Training Data} & \multicolumn{2}{|c|}{Dev} & \multicolumn{2}{|c|}{Test} \\ \hline
\multicolumn{1}{|c|}{Data Source} & Year & All & Low & All & Low   \\ \hline
%ST & \multicolumn{1}{|c|}{Cos} & 34.6 & 40.6 & 24.5 & 17.8 \\ \hline

\multicolumn{1}{|c|}{SMTeuroparl}&	2012&63.5&41.7&49.6&43.3 \\
\multicolumn{1}{|c|}{surprise.SMTnews}&	2012&67.1&49.2&58.4&56.5 \\
\multicolumn{1}{|c|}{postediting}&	2016&70.3&53.9&60.5&56.3 \\
\multicolumn{1}{|c|}{tweet-news}&	2014&68.8&52.4&61.4&57.1 \\
\multicolumn{1}{|c|}{answers-students}&	2015&67.5&53.1&62.5&56.4 \\
\multicolumn{1}{|c|}{headlines}&	2014&69.2&52.8&62.6&53.8 \\
\multicolumn{1}{|c|}{plagiarism}&	2016&72.1&59.5&65.4&62.4 \\
\multicolumn{1}{|c|}{belief}&	2015&71.9&53.5&65.7&59.1 \\
\multicolumn{1}{|c|}{FNWN}&	2013&71.2&54.7&67.1&61.9 \\
\multicolumn{1}{|c|}{headlines}&	2015&73.8&58.9&67.9&53.1 \\
\multicolumn{1}{|c|}{question-question}&	2016&75.0&63.2&69.3&65.5 \\
\multicolumn{1}{|c|}{OnWN}&	2013&\textbf{75.9}&63.4&70.3&64.0 \\
\multicolumn{1}{|c|}{OnWN}&	2014&74.9&\textbf{63.5}&70.6&\textbf{65.6} \\
\multicolumn{1}{|c|}{surprise.OnWN}&	2012&75.5&57.5&\textbf{71.5}&60.6 \\ \hline
\multicolumn{2}{|c|}{Average}	&71.2&55.5&64.5&58.2 \\ \hline

\end{tabular}
}
\centering
\caption{The Pearson correlation (\%) of sentence-BERT on STS benchmark. The sentence-BERT is initialized by the BERT base model and trained by 100 samples in each data source. All results are the average of three runs. The order of rows is determined by their performance on the test set of STSB.}
\label{tb:sentence_bert_details}
\end{table}

%most of the sentence pairs are highly similar with each other.
%The other baselines are just for showing that Glove + weighted performs well compared with other alternative

%Do not provide +SIF because of the lack of training and testing split












\subsection{Summarization Comparison Given the Same Summary Length}
\label{sec:sum_more}

In Section~\refsum%~\ref{sec:sum}
, we compare our methods with other baselines when all the methods choose the same number of sentences. We suspect that the bad performances for \textbf{W Emb (*)} methods (i.e., representing each sentence using the embedding of words in the sentence) might come from the tendency of selecting shorter sentences.
%\footnote{In our implementation, we define the similarity between each word and an empty set of embeddings from sentences as -1000, so \textbf{W Emb (*)} nearly always choose the shortest sentence when selecting the first sentence.} 
To verify the hypothesis, we plot the R-1 performance of different unsupervised summarization methods that do not use the sentence order information versus the sentence length in Figure~\ref{fig:summarization}. 

In the figure, we first observe that \textbf{Ours (K=100)} significantly outperforms \textbf{W Emb (GloVe)} and \textbf{Sent Emb (GloVe)} when summaries have similar length. In addition, we find that \textbf{W Emb (*)} usually outperforms \textbf{Sent Emb (*)} when comparing the summaries with a similar length. Notice that this comparison might not be fair because \textbf{W Emb (*)} are allowed to select more sentences given the same length of summary and it might be easier to cover more topics in the document using more sentences. In practice, preventing choosing many short sentences might be preferable in an extractive summarization if fluency is an important factor.

Nevertheless, suppose our goal is simply to maximize the ROUGE F1 score given a fixed length of the summary without accessing the ground truth summary and sentence order information. In that case, the figure indicates that \textbf{Ours (K=100)} significantly outperform \textbf{W Emb (GloVe)} and is the best choice when the summary length is less than around 50 words and \textbf{W Emb (BERT)} becomes the best method for a longer summary. The BERT in this figure is the BERT base model. The mixed results suggest that combining our method with BERT might be a promising direction to get the best performance in this task (e.g., use contextualized word embedding from BERT as our pre-trained word embedding space). 




\begin{figure}[t!]
\begin{center}
\includegraphics[width=1\linewidth]{figures/summarization_results_new.pdf}
\end{center}
\caption{Comparing the F1 of ROUGE-1 score on unsupervised methods that do not access the sentence order information in CNN/Daily Mail.}
\label{fig:summarization}
\end{figure}


\begin{table*}[t!]
\scalebox{1}{
\begin{tabular}{|cc|c|cc|cc|}
\hline
 & & \multicolumn{3}{|c|}{Lowercase} & \multicolumn{2}{|c|}{Uppercase}  \\ \hline %\cline{1-2}
\multicolumn{2}{|c|}{Method} & BiRD & WikiSRS-Sim & WikiSRS-Rel & WikiSRS-Sim & WikiSRS-Rel  \\ \hline %\cline{1-2}
\multicolumn{1}{|c|}{Model} & Score & Pearson & \multicolumn{4}{|c|}{Spearman}  \\ \hline
%\multirow{2}{*}{BERT} & \multicolumn{1}{|c|}{CLS} & 54.7 & 66.7 & 29.2 & 15.5 & 17.2 & 5.4 & 4.2 \\ 
ELMo & \multicolumn{1}{|c|}{Avg} &  - & - & - & 54.4 &	49.2  \\ 
BERT & \multicolumn{1}{|c|}{Avg} &  44.4 & 43.3 & 40.7 & 40.3 & 37.8  \\ 
GloVe & \multicolumn{1}{|c|}{Avg}  & 47.9\footnotemark & 47.7 & 49.1 & 62.7 &	62.7 \\ 
Ours (K=10) & \multicolumn{1}{|c|}{Emb} & 57.3 & \textbf{67.4} & \textbf{66.9} & 68.6 & \textbf{69.6} \\ 
Ours (K=1) & \multicolumn{1}{|c|}{Emb} & \textbf{60.6} & 67.1 & 65.8 & \textbf{69.4} &	69.4 \\ \hline
\end{tabular}
}
%$\dagger$The results are taken from~\citet{WikiSRS}.   }
\centering
\caption{Performances of phrase similarity tasks. In BiRD and WikiSRS, the correlation coefficient (\%) between the predicted similarity and the ground truth similarity is presented. }
\label{tb:phrase_sim_more}
\end{table*}

\begin{table}[t!]
\scalebox{0.8}{
\begin{tabular}{|cc|c|c|}
\hline
\multicolumn{3}{|c|}{Similarity} & Summarization  \\ \hline
\multicolumn{2}{|c|}{STSB All} & STS2012-6 All & CNN DM  \\	
Dev & Test & Test& Dev   \\
1,500 & 1,379 & 12,544 & 11,490  \\ \hline
\end{tabular}
}
\centering
\caption{Dataset sizes for sentence representations.}
\label{tb:dataset_size_sent}
\end{table}

\begin{table}[t!]
\scalebox{0.8}{
\begin{tabular}{|c|c|c|cc|cc|}
\hline
\multicolumn{5}{|c|}{Similarity} & \multicolumn{2}{|c|}{Hypernym} \\ \hline
SemEval 2013 & Turney2012 & BiRD & \multicolumn{2}{|c|}{WikiSRS} & \multicolumn{2}{|c|}{HypeNet}	\\
Test & Test & Test &Sim & Rel & Val & Test \\
7,814 & 1,500 & 3,345 &688 & 688 & 3,534 & 17,670 \\ \hline
\end{tabular}
}
\centering
\caption{Dataset sizes for phrase representations.}
\label{tb:dataset_size_phrase}
\end{table}



\subsection{Experiments on More Phrase Similarity Datasets}
\label{sec:phrase_sim_more}
We conduct the phrase similarity experiments on two recently proposed datasets, BiRD~\citep{bird-naacl2019}, and WikiSRS~\citep{WikiSRS}, which contain ground truth phrase similarities derived from human annotations. BiRD and WikiSRS-Rel measure the relatedness of phrases and WikiSRS-Sim measures the similarity of phrases. The phrases are proper nouns in WikiSRS and are mostly common nouns in BiRD. Since the main goal of WikiSRS is to test the entity representation, we also test the different models trained on the corpus without lowercasing all the words. 

The results are presented in Table~\ref{tb:phrase_sim_more}. The multi-facet embedding performs similarly compared with single-facet embedding and is better than other baselines. This result confirms our findings in the main paper that the phrase similarity performance is not sensitive to the number of clusters $K$.

\input{BERT_large}

\input{motivations}


\subsection{Comparison with BERT Large}
\label{sec:bert_large}
In Table~\ref{tb:model_size}, we compare the size and running time of different models for sentence representation. As mentioned in Section~\refexpsetup%~\ref{sec:exp}
, our model has fewer parameters than the BERT base model and uses much fewer computational resources for training, so we only present the BERT Base performance in the experiment sections. Nevertheless, we still wonder how well BERT large can perform in these unsupervised semantic tasks, so we compare our method with BERT Large in Table~\ref{tb:STS_bert}, Table~\ref{tb:sum_bert}, Table~\ref{tb:phrase_sim_bert}, Table~\ref{tb:phrase_hyper_bert}. As we can see, BERT large is usually better than BERT base in the similarity tasks but performs worse in the hypernym detection task. The BERT's performance gains in similarity tasks might imply that training a larger version of our model might be a promising future direction. %Although increasing the model size boosts the performance of BERT, our method is still better in most of the cases. 
%, and Table~\ref{tb:sent_entail_bert}
%, especially in the phrase similarity tasks
%One of the main reasons we hypothesize is that BERT is trained by predicting the masked words in the input sequence and the objective function might not be good if sequences are short (like phrases). 



\subsection{Motivating Examples in Sentence Similarity}
\label{sec:good_example_STS}

In order to further understand when and why our methods perform well, we present some sentences pairs from the MSRvid dataset in STS 2012 in Table~\ref{tb:good_example_STS} and~\ref{tb:good_topics_STS} on which our methods perform well. 

In Table~\ref{tb:good_example_STS}, the first two sentence pairs have relatively high similarities but a lower ratio of overlapping words, so the baseline based on average word embedding (i.e., \textbf{Avg}) underestimates the similarities. Softly removing the stop words (i.e., \textbf{Prob\_avg}) alleviates the problem, but the inverse frequency of words do not completely align with the importance of words in the sentences. 

We visualize our predicted word importance and codebook embeddings in Table~\ref{tb:good_topics_STS}. Combining the estimated word importance with the inverse word frequency (i.e., \textbf{Prob\_avg + Our a}) improves the performance. Finally, computing the similarity between the codebook embeddings (i.e., \textbf{Our c}) leads to the best results. The reason of the improvement might be that the unimportant words in the sentence often do not significantly affect the co-occuring word distribution. Take the second sentence pair as an example, mentioning \emph{``with the big eyes''} does not change the sentence's meaning and facets too much.
%This is because although the sentences using different word choices or using extra words to describe the details, the distribution of possible words in the nearby sentences is similar. Take the first sentence pair as an example, appending "in the garage" after "A man is lifting weights" does not significantly change the existing aspects of the sentences.

On the contrary, the last sentence pair in Table~\ref{tb:good_example_STS} has a low similarity but relatively higher word overlapping. Our model could infer that \emph{riding a horse} is very different from \emph{riding an elephant} because their co-occurring word distributions are different. The appearance of \emph{riding a horse} implies that we are more likely to observe a race topic in nearby sentences, but \emph{riding an elephant} increases the chance of seeing a movie topic instead.
%In the predicted codebook embeddings, we can see that riding horse 

%Weighting the words using  
%our methods rank the first three sentence pairs higher than the baselines do.

%The first three sentences pairs 
%Table


\footnotetext{The number is different from the one reported in \citet{bird-naacl2019} because we use the uncased version (42B), the embedding space our model is trained on, and they use the cased version (840B).}

\subsection{Motivating Examples in Extractive Summarization}
\label{sec:good_example_sum}

In Table~\ref{tb:good_example_sum}, we show the top three sentences that different methods choose to summarize a story about a photographer, Erik Johansson, and his artwork.

In this document, \textbf{Lead-3} does not cover its main points because this article starts with a preamble. Our method selects the first sentence as a good summary because it highlights the main character of the story, Erik Johansson, and his art style. The selected sentences contain the aspects that cover several topics in the whole document.
%The first sentence our method selects serves 

Average word embedding baselines, \textbf{Sent\_Emb (GloVe)} and \textbf{Sent\_Emb (BERT)}, select the sentences that focus on describing how his artwork is created. Nevertheless, the sentences are hard to understand without the context in the article. We hypothesize that the methods tend to avoid selecting the sentences with diverse aspects because after averaging the word embeddings, the resulting single embedding is not close to the embedding of words in the documents.

Finally, \textbf{W\_Emb (GloVe)} and \textbf{W\_Emb (BERT)} tend to select shorter sentences because we normalize the objective function by the sentence lengths. It is hard to remove the bias of selecting shorter or longer sentences because each sentence is represented by a different number of embeddings.

%summarize the whole document well.
%The second sentence describes one of his artworks and the third one emphasize that his art creates.
%Then, the rest of two selected sentences

%confuses when there are several aspects in the sentence. Normalized GloVe embeddings method tends to select short sentences. Methods based on BERT select a sentence cited in the ground truth, but the sentence is actually hard to understand without the context in the article.




==> AAAI 2021 NSD/motivations.tex <==
\begin{table*}[t!]
\scalebox{0.85}{
\begin{tabular}{|cc|c|ccccc|}
\hline
\multirow{2}{*}{Sentence 1} & \multirow{2}{*}{Sentence 2} & Score & \multicolumn{5}{|c|}{Score Rank Among 1500 Pairs} \\
 &  & GT & GT & Our c & Prob\_avg + Our a  & Prob\_avg & Avg \\ \hline
%A man is lifting weights in a garage . &  A man is lifting weights . & 4.25 & 165 & 213 & 226 & 316 & 398 \\ 
A turtle walks over the ground . & A large turtle crawls in the grass . & 3.75 & 326 & 400 & 638 & 717 & 761 \\
The animal with the big eyes is eating . & A slow loris is eating . & 2.60 & 690 & 611 & 1001 & 1223 & 1370 \\
A man is riding on a horse . & A woman is riding an elephant . & 1.53 & 1021 & 869 & 722 & 549 & 540 \\ \hline
%\multicolumn{2}{|c|}{\colorbox{c79}{A} \colorbox{c27}{man} \colorbox{c50}{is} \colorbox{c21}{lifting} \colorbox{c23}{weights} \colorbox{c58}{in} \colorbox{c49}{a} \colorbox{c45}{garage} \colorbox{c63}{.}} & \multicolumn{6}{|c|}{\colorbox{c83}{A} \colorbox{c41}{man} \colorbox{c56}{is} \colorbox{c07}{lifting} \colorbox{c10}{weights} \colorbox{c66}{.}}  \\ \hline
\end{tabular}
}
\centering
\caption{Motivating examples for a sentence similarity task. The sentences are image captions from MSRvid dataset in STS 2012. GT means ground truth. All our methods here set $K=10$.}
\label{tb:good_example_STS}
\end{table*}

\begin{table*}[t!]
\scalebox{0.95}{
\begin{tabular}{|c|c|c|}
\hline
& Sentence 1 & Sentence 2 \\ \hline
% Sentences &\colorbox{c79}{A} \colorbox{c27}{man} \colorbox{c50}{is} \colorbox{c21}{lifting} \colorbox{c23}{weights} \colorbox{c58}{in} \colorbox{c49}{a} \colorbox{c45}{garage} \colorbox{c63}{.} & \colorbox{c83}{A} \colorbox{c41}{man} \colorbox{c56}{is} \colorbox{c07}{lifting} \colorbox{c10}{weights} \colorbox{c66}{.}  \\ \hline
% & can 0.872 even 0.851 should 0.850 & can 0.865 either 0.843 should 0.841 \\
% & front 0.762 bottom 0.742 down 0.714 & front 0.758 bottom 0.758 sides 0.691  \\
% & lifting 0.866 lift 0.663 Lifting 0.621 & lifting 0.847 lift 0.635 Lifting 0.610   \\
% & garage 0.876 garages 0.715 basement 0.707 & lifting 0.837 lift 0.652 weights 0.629   \\
% Predicted& decreasing 0.677 decreases 0.655 negligible 0.649 & decreasing 0.709 decreases 0.685 increases 0.682  \\
% Embeddings& weights 0.883 Weights 0.678 weight 0.665 & weights 0.864 weight 0.700 Weights 0.646  \\
% & cylindrical 0.700 plurality 0.675 axial 0.674 & annular 0.738 cylindrical 0.725 circumferential 0.701  \\
% & configurations 0.620 incorporating 0.610 utilizing 0.605 & methods 0.612 configurations 0.610 graphical 0.598  \\
% & man 0.872 woman 0.682 men 0.672 & sweating 0.498 cardiovascular 0.494 dehydration 0.485  \\
% & man 0.825 men 0.671 woman 0.653 & man 0.888 woman 0.690 men 0.676 \\ \hline
Sentences & \colorbox{c83}{A} \colorbox{c22}{turtle} \colorbox{c41}{walks} \colorbox{c42}{over} \colorbox{c45}{the} \colorbox{c18}{ground} \colorbox{c61}{.} & \colorbox{c82}{A} \colorbox{c36}{large} \colorbox{c32}{turtle} \colorbox{c61}{crawls} \colorbox{c60}{in} \colorbox{c52}{the} \colorbox{c28}{grass} \colorbox{c64}{.} \\ \hline
& can 0.876 you 0.846 even 0.845 & can 0.857 even 0.838 often 0.832 \\
& turtle 0.914 turtles 0.822 dolphin 0.755 & turtle 0.917 turtles 0.818 dolphin 0.755 \\
& hillside 0.737 hills 0.711 mountains 0.704 & beneath 0.697 hillside 0.645 down 0.639 \\
& species 0.937 habitat 0.771 habitats 0.759 & species 0.949 habitat 0.778 habitats 0.760  \\
Output & animals 0.689 pigs 0.675 animal 0.658 & females 0.655 males 0.630 male 0.622  \\
Embeddings& white 0.842 blue 0.839 red 0.833 & white 0.863 blue 0.862 red 0.856  \\
& insectivorous 0.650 immatures 0.627 insectivores 0.618 & immatures 0.616 foliose 0.609 tussocks 0.607  \\
& ground 0.693 soil 0.676 surface 0.626 & seawater 0.644 salinity 0.597 soils 0.593 \\
& ground 0.861 grass 0.598 Ground 0.576 & grass 0.870 grasses 0.739 weeds 0.713   \\
& waking 0.551 strolls 0.551 wander 0.546 & length 0.732 width 0.639 diameter 0.627  \\ \hline
Sentences & \colorbox{c82}{The} \colorbox{c24}{animal} \colorbox{c56}{with} \colorbox{c54}{the} \colorbox{c51}{big} \colorbox{c31}{eyes} \colorbox{c58}{is} \colorbox{c28}{eating} \colorbox{c66}
{.} & \colorbox{c84}{A} \colorbox{c47}{slow} \colorbox{c64}{loris} \colorbox{c62}{is} \colorbox{c27}{eating} \colorbox{c65}{.} \\ \hline
& even 0.887 sure 0.877 want 0.868 & often 0.880 usually 0.860 sometimes 0.838 \\
& animals 0.896 animal 0.896 rabbits 0.678 & loris 0.864 lorises 0.670 langur 0.596   \\
& food 0.825 foods 0.802 eating 0.798 & foods 0.763 food 0.709 nutritional 0.690 \\
& fingers 0.695 legs 0.692 shoulders 0.691 & eating 0.799 food 0.798 eat 0.794 \\
Output & species 0.919 habitats 0.738 habitat 0.731 & species 0.949 habitat 0.787 habitats 0.769 \\
Embeddings & blue 0.834 red 0.809 white 0.805 & blue 0.844 white 0.839 red 0.827 \\
& ingestion 0.608 inflammation 0.591 concentrations 0.588 & gently 0.649 wet 0.642 beneath 0.641\\
& male 0.652 female 0.636 disease 0.618 & male 0.685 female 0.659 females 0.658  \\
& profound 0.668 perceived 0.647 profoundly 0.634  &  decreasing 0.710 decreases 0.699 decrease 0.697  \\
& beady 0.626 beaks 0.623 mandibles 0.602 & C. 0.624 L. 0.620 A. 0.593   \\ \hline
Sentences& \colorbox{c78}{A} \colorbox{c21}{man} \colorbox{c52}{is} \colorbox{c27}{riding} \colorbox{c67}{on} \colorbox{c52}{a} \colorbox{c16}{horse} \colorbox{c66}{.} & \colorbox{c80}{A} \colorbox{c14}{woman} \colorbox{c50}{is} \colorbox{c33}{riding} \colorbox{c57}{an} \colorbox{c16}{elephant} \colorbox{c67}{.} \\ \hline
& sure 0.883 even 0.883 want 0.867 & sure 0.880 even 0.876 know 0.866 \\
& slid 0.686 legs 0.681 shoulders 0.670 & underneath 0.701 shoulders 0.671 legs 0.668  \\
& moisture 0.518 drying 0.517 coated 0.516 & elephant 0.912 elephants 0.842 hippo 0.759  \\
& horse 0.917 horses 0.878 stallion 0.728 & elephant 0.885 elephants 0.817 animals 0.728   \\
Output & mortals 0.668 fearful 0.664 beings 0.646 & fearful 0.677 disdain 0.637 anguish 0.632  \\
Embeddings & man 0.864 woman 0.764 boy 0.700 & woman 0.822 women 0.787 female 0.718 \\
& man 0.858 woman 0.652 boy 0.637 & girl 0.784 woman 0.781 lady 0.721  \\
& discovers 0.647 informs 0.638 learns 0.634 & discovers 0.662 learns 0.659 realizes 0.648 \\
& race 0.812 races 0.800 championship 0.697 & movie 0.622 film 0.615 films 0.590  \\
& Horse 0.763 Riding 0.696 Horses 0.656 & riding 0.873 bike 0.740 biking 0.731  \\ \hline
\end{tabular}
}
\centering
\caption{The predicted word importance and codebook embeddings on sentences from Table~\ref{tb:good_example_STS}. The way of visualization is the same as that in
Section~\ref{sec:more_examples}.
}
\label{tb:good_topics_STS}
\end{table*}

\begin{table*}[t!]
\scalebox{0.75}{
\begin{tabular}{|c|c|p{19cm}|}
\hline
Method & Index & \multicolumn{1}{|c|}{Selected Sentence} \\ \hline
 & NA & Swedish photographer , Erik Johansson , spends months photographing images to build up to the finished picture . \\
Ground Truth & NA & Each image is made up of hundreds of separate shots and painstakingly detailed work by the expert retoucher . \\
& NA & Erik , 30 , said : ' Can I put this very weird idea in a photograph and make it look like it was just captured ? ' \\ \hline
 & 1 & Thought the black and blue dress was an optical illusion ? \\
Lead-3 & 2 & It 's nothing compared to these mind - boggling pictures by a Swedish photographer , artist , and Photoshop genius . \\
 & 3 & Erik Johansson , 30 , who is based in Berlin , Germany , says he does n’t capture moments , but instead captures ideas . \\ \hline
 & 6 & Swedish photographer , artist , and Photoshop genius , Erik Johansson , has created mind - boggling photos like this inside - out house that look different on each glance . \\
Our c (K=10) & 42 & Reverse Opposite is mind - bendig as , with an MC Escher drawing , the car seems both on and under the bridge at the same time . \\
& 1 & Thought the black and blue dress was an optical illusion ? \\
\hline
 & 46 & Although one photo can consist of lots of different images merged into one , he always wants it to look like it could have been captured as a whole picture . \\
\multirow{2}{*}{Sent\_Emb (GloVe)} & 25 & He cites Rene Magritte , Salvador Dali and MC Escher as artistic influences . \\
 & 18 & Using Photoshop , he turned the running paint into rolling fields and superimposed a photograph of a house on to the cardboard model , adding a photo of a water wheel to complete the fantastical and dramatic shot of a dreamy , bucolic landscape that seems to be falling over a cliff . \\ \hline
 & 41 & he said . \\
W\_Emb (GloVe) & 23 & But there are tons of inspiration online . \\
& 22 & ' I think I get more inspiration from paintings rather than photos . \\ \hline
\multirow{5}{*}{Sent\_Emb (BERT)} & 18 & Using Photoshop , he turned the running paint into rolling fields and superimposed a photograph of a house on to the cardboard model , adding a photo of a water wheel to complete the fantastical and dramatic shot of a dreamy , bucolic landscape that seems to be falling over a cliff . \\
 &41 & he said . \\
&12 & He said : ' It ’s the challenge : can I put this very weird idea in a photograph and make it look like it was just captured ? ' \\ \hline
 &5 & Scroll down for video . \\
W\_Emb (BERT) & 30 & In Closing Out , interiors and exterior meld as one in this seemingly simple tableau . \\
 & 12 & He said : ' It ’s the challenge : can I put this very weird idea in a photograph and make it look like it was just captured ? ' \\ \hline
\end{tabular}
}
\centering
\caption{Motivating examples for extractive summarization. The sentences come from a document in the validation set of CNN/Daily Mail. Index indicates the sentence order in the document. Ground truth means the summary from humans. The sentences in each method are ranked by its selection order. For example, our method selects the $6$th sentence in the document first.}
\label{tb:good_example_sum}
\end{table*}

==> AAAI 2021 NSD/related_work.tex <==


Topic modeling~\citep{blei2003latent} has been extensively studied and widely applied due to its interpretability and flexibility of incorporating different forms of input features~\citep{MimnoM08}. 
%Extensions of the topic models are able to  
\citet{cao2015novel, SrivastavaS17} demonstrate that neural networks could be applied to discover semantically coherent topics. Instead of optimizing a global topic model, our goal is to efficiently discover different sets of topics/clusters on the words beside each (unseen) phrase or sentence.

Recently, \citet{gupta2019improving} and \citet{gupta2020p} discover that global clustering could improve the representation of sentences and documents. In our work, we show that a local clustering could be used in several downstream applications, including word importance estimation for measuring sentence similarity. Whether combining global clustering and local clustering could lead to a further improvement is an interesting future research direction.

Sparse coding on word embedding space is used to model the multiple facets of a word~\citep{faruqui2015sparse,arora2018linear}, and parameterizing word embeddings using neural networks is used to test hypothesis~\citep{HanGSC18} and save storage space~\citep{ShuN18}. Besides, to capture asymmetric relations such as hypernyms, words are represented as single or multiple regions in Gaussian embeddings~\citep{VilnisM15, athiwaratkun2017multimodal} rather than a single point. However, the challenges of extending these methods to longer sequences are not addressed in these studies.

One of our main challenges is to design a loss for learning to predict cluster centers while modeling the dependency among the clusters. This requires a matching step between two sets and computing the distance loss after the matching~\citep{eiter1997distance}. One popular loss is called Chamfer distance, which is widely adopted in the auto-encoder models for point clouds~\citep{yang2018foldingnet, liu2019l2g}, while more sophisticated matching loss options are also proposed~\citep{stewart2016end, balles2019holographic}. The goal of the previous studies focuses on measuring symmetric distances between the ground truth set and predicted set (usually with an equal size), while our loss tries to reconstruct the ground truth set using much fewer codebook embeddings. 

Other ways to achieve the permutation invariant loss for neural networks include sequential decision making~\citep{WelleckYGMZC18}, mixture of experts~\citep{yang2018breaking, wang2019attention}, beam search~\citep{label_set}, predicting the permutation using a CNN~\citep{rezatofighi2018deep}, Transformers~\citep{stern2019insertion, gu2019insertion, carion2020} or reinforcement learning~\citep{welleck2019non}. In contrast, our goal is to efficiently predict a set of cluster centers that can well reconstruct the set of observed instances rather than directly predicting the observed instances.

%removing the elements in the ground truth set which have been predicted

%Several set encoder models have been proposed~\citep{vinyals2015order, zaheer2017deep, lee2018set, murphy2018janossy}, but relatively fewer studies explore how to decode a set or allow the decoder to learn its own order of prediction. 

%The goals of these work are predicting or reconstruct 


%exploring all possible permutations~\citep{vinyals2015order},

%does not discuss how to extending these methods to represent .

%When learning word embeddings, 
%, Gaussian embeddings~ represent each word as a . 

%compress the word embeddings
%save space for conditional embeddings

%\citep{HanGSC18} (Conditional Word Embedding and Hypothesis Testing via Bayes-by-Backprop)
%\citep{ShuN18} (Compressing Word Embeddings via Deep Compositional Code Learning)



%\citep{dieng2016topicrnn}

%Single word or document embedding based on autoencoders
%\citep{lauly2017document} (DocNADE) 
%\citep{amiri2016learning}


%set encoder


